Evaluating Blocking Biases in Entity Matching

Entity Matching (EM) is crucial for identifying equivalent data entities across different sources, a task that becomes increasingly challenging with the growth and heterogeneity of data. Blocking techniques, which reduce the computational complexity of EM, play a vital role in making this process scalable. Despite advancements in blocking methods, the issue of fairness; where blocking may inadvertently favor certain demographic groups; has been largely overlooked. This study extends traditional blocking metrics to incorporate fairness, providing a framework for assessing bias in blocking techniques. Through experimental analysis, we evaluate the effectiveness and fairness of various blocking methods, offering insights into their potential biases. Our findings highlight the importance of considering fairness in EM, particularly in the blocking phase, to ensure equitable outcomes in data integration tasks.

==> extensions.tex <==
\section{$(k,\Sigma)$-Anonymization with Generalization}
\fei{Shall we remove this section, and maybe mention the idea in Conclusion as future work?}
So far we studied $(k,\Sigma)$-anonymization with suppression as the anonymization process. Now, we extend $(k,\Sigma)$-anonymization with generalization. Generalization is an anonymization process that replaces values in a private table with less specific, but semantically consistent values according to a generalization hierarchy~\cite{IYENGARV.S.2002,SAMARATIP.2001,SWEENEYL.2002a, SWEENEYL.2002b,SWEENEYL.1998}. To generalize attribute $A$, we assume a set of levels $\mc{L}^A=\{l^A_0,...,l^A_h\}$ and a partial order $\le^A$, called a {\em generalization relation} on $\mc{L}^A$. Levels $l^A_i$ are assigned with disjoint domain-sets $\dom(l^A_i)$. In $\le^A$, each level has at most one parent. The domain-set $\dom(l^A_n)$ is the maximal domain set and it is a singleton, and $\dom(l^A_0)$ is the {\em ground domain set}. The definition of $\le^A$ implies the existence of a totally ordered hierarchy, called the {\em domain generalization hierarchy}, $\dgh^A$. The domain set $\dom(l^A_i)$ generalizes $\dom(l^A_j)$ iff $l^A_j \leq l^A_i$. We use $h^A$ to refer to the number of levels in $\dgh^A$\ignore{, i.e. $h^A=|\mc{L}^A|$}. 

\begin{figure}[h]
    \centering
    \vspace{-2mm}
    \includegraphics[width=6cm]{./figs/age}
    \vspace{-3mm}
    \caption{(a) \dgh \ and (b) \vgh \ for \att{AGE}.}
    \label{fig:age}
    \vspace{-3mm}
\end{figure}


\begin{definition} [Diversity Constraints with Generalization] \label{df:div-gen} Given a ground relation $R$ with schema $\mc{R}=\{A_1,...,A_n\}$ and generalization hierarchies $\mc{L}^{A_i}$ for each attribute $A_i$, a diversity constraint is a pair $(\sigma,d)$ in which $\sigma$ is a diversity constraint $\nit{floor}\le A_i(a) \le \nit{ceil}$ as in Definition~\ref{df:div} and $d$ is a distance value for values in $\mc{L}^{A_i}$ attribute. A relation $R'$ that generalizes the ground relation $R$ satisfies $\sigma$, denoted by $R' \models \sigma$, if $\nit{floor}\le |\{t\;|\;t \in R', \delta(t[A_i],a) \le d\}| \le \nit{ceil}$. \end{definition}

This means the number of tuples $t$ in $R'$ with value $t[A_i]$ in the distance $d$ of $a$ is at least \nit{floor} and at most \nit{ceil}. The diversity constraints with value generalization extends the diversity constraints with suppression using the distance value $d$ that is a threshold for closeness to a value $a$ to be preserved. 

\fei{This is interesting, but not clear how to incorporate into the algorithm, and also the foundations.  With the above, this sounds more like a starting discussion for future work, where we can define diversity constraints with generalization, and we list the next steps and challenges.}




==> extras.tex <==
\ignore{An ideal blocking technique is one where $\candidatePairs = \equivPairs$, resulting in $\PC = \PQ = 1$ and the $\RR = 1 - \frac{|\equivPairs|}{|\pairs|}$. We refer to this specific \RR as $\RR_{opt}$. To combine these metrics into a single, unified measure, we draw inspiration from machine learning. We propose \(F_{\PQ,\PC}\), analogous to the F1-score in machine learning, which is the harmonic mean of \PC and \PQ, as shown in Eq. \eqref{eq:f_score}:

\begin{align}
    F_{\PQ,\PC} = \frac{2 \times \PC \times \PQ}{\PC + \PQ}\label{eq:f_score}
\end{align}

Additionally, we introduce the Normalized Reduction Ratio Deviation \NRRD to capture the deviation of \RR from \(\RR_{opt}\). It is defined as follows:

\begin{align}
\NRRD(\RR, \RR_{opt}) = 1 - \sqrt{\frac{\left|\RR - \RR_{opt}\right|}{\max\left(1 - \RR_{opt}, \RR_{opt}\right)}}
\end{align}

The \NRRD metric ranges from 0 to 1, attaining a value of 1 when \RR equals \(\RR_{opt}\), and a value of 0 when \RR is at either extreme (0 or 1). The use of the max function ensures that the normalization is appropriate for scenarios where \(\RR_{opt}\) is less than 0.5 or greater than 0.5.

Finally, we define the Pareto Blocker Score (\PBS), which integrates all these metrics into a single score:

\begin{align}
       \PBS = \sqrt{F_{\PQ,\PC} \times \NRRD(\RR, \RR_{opt})}
\end{align}

The \PBS score ranges from 0 to 1, with the objective being to maximize this score, ideally approaching 1. Figure~\ref{fig:PBS} illustrates the behavior of the \PBS metric, underscoring the importance of optimizing both the \RR and \(F_{\PQ,\PC}\) to achieve the highest \PBS. This effectively demonstrates the utility of the \PBS metric in evaluating the performance of blocking methods. This metric is inspired by the work presented by ~\cite{o2018new}, where a new metric was introduced to capture \PC, \PQ, and runtime. Inspired by their logic, we defined the \PBS to incorporate \PC, \PQ, and \RR.

\begin{figure}
         \centering
         \subfloat[\PBS vs $F_{\PQ,\PC}$]{\label{fig:PBS-F}
			{\includegraphics[width=0.23\textwidth]{figs/PBS-F.pdf}}}
		\subfloat[\PBS vs \RR]{\label{fig:PBS-RR}
			{\includegraphics[width=0.23\textwidth]{figs/PBS-RR.pdf}}}	
			% \vspace{-3mm}
	
 \caption{Fig. ~\ref{fig:PBS-F} shows that the \PBS score reaches its peak when \RR is equal to the $\RR_{opt}$, especially for higher values of \(F_{PQ,PC}\). Fig. ~\ref{fig:PBS-RR} illustrates that \PBS increases with \(F_{PQ,PC}\) and achieves higher values when \RR is closer to $\RR_{opt}$. 
}\label{fig:PBS}
\end{figure}}





% The goal of the experiments conducted in this study is to evaluate the performance of various prominent blocking methods across different datasets, with a specific focus on measuring the \RR, \PC, and \PQ for both majority and minority subgroups. By calculating these metrics for each group, the experiments aim to quantify the disparities in blocking performance and assess the fairness of these methods.

% We utilize datasets from well-established EM benchmarks~\cite{mudgal2018deep}: Walmart-Amazon, Beer, Amazon-Google, Fodors-Zagat, iTunes-Amazon, DBLP-Google Scholar, DBLP-ACM, and Febrl~\cite{mudgal2018deep,yang2020fairness}. These datasets are widely used in the research community for evaluating the performance of EM systems.

% In our analysis, entities are categorized into minority and majority groups based on specific sensitive attributes identified within each dataset, as outlined in Table~\ref{tab:datasets}. For example, in the Walmart-Amazon dataset, entities categorized under ``printers'' within the ``category'' attribute are classified as the minority group. In the Beer dataset, the ``Beer\_Name'' attribute's inclusion of ``Red'' identifies the minority group. Similarly, in Amazon-Google, entities with ``Microsoft'' as the ``manufacturer'' are considered part of the minority group. The Fodors-Zagat dataset designates entities with the ``type'' attribute labeled as ``Asian'' as the minority. In iTunes-Amazon, the minority group is composed of entities labeled as ``Dance'' within the ``Genre'' attribute. For DBLP-Google Scholar, the minority group is identified by the presence of ``vldb j'' in the ``venue'' attribute, while in DBLP-ACM and Febrl, entities are considered part of the minority if the ``authors'' or ``given\_name'' attribute includes a female name.




\ignore{\small 
\begin{table}
    \centering
    \begin{tabular}{*{4}{l}} 
    \toprule
        \textbf{Dataset} & 
        \textbf{\# Attr.} & 
        \textbf{\# Matching Pairs} & 
        \textbf{Total Records} \\
    \midrule
        \walamz & 
        5 & 
        962 & 
        24,628 \\
        \Beer & 
        4 & 
        68 & 
        7,345 \\
        \amzgog & 
        3 & 
        1,167 & 
        4,589 \\
        \FodorZag & 
        6 & 
        110 & 
        864 \\
        \itunamz & 
        8 & 
        132 & 
        62,830 \\
        \DBLPGogS & 
        4 & 
        5,347 & 
        66,879 \\
        \DBLPACM & 
        4 & 
        2,220 & 
        4,910 \\
        \Febrl & 
        7 & 
        8,520 & 
        12,983 \\
    \bottomrule
    \end{tabular}
    \caption{Datasets and their characteristics.\mhm{fix this later}}
    \vspace{-2mm}
    \label{tab:datasets}
\end{table}
}




% {\small 
% \begin{table*}
%     \centering
%     \begin{tabular}{*{7}{l}} 
%     \toprule
%         \textbf{Dataset} &
%         \textbf{Domain} & 
%         \textbf{\# Attr.} & 
%         \textbf{\# Matching Pairs} & 
%         \textbf{Total Records} &
%         \textbf{Sensitive Attribute} &
%         \textbf{Sensitive Value} \\
%     \midrule
%         Walmart-Amazon &
%         Electronics & 
%         5 & 
%         962 & 
%         24,628 & 
%         Category & 
%         Printers \\
%         Beer &
%         Beer & 
%         4 & 
%         68 & 
%         7,345 & 
%         Beer\_Name & 
%         Red \\
%         Amazon-Google &
%         Software & 
%         3 & 
%         1,167 & 
%         4,589 & 
%         Manufacturer & 
%         Microsoft \\
%         Fodors-Zagat &
%         Restaurant & 
%         6 & 
%         110 & 
%         864 & 
%         Type & 
%         Asian \\
%         iTunes-Amazon &
%         Music & 
%         8 & 
%         132 & 
%         62,830 & 
%         Genre & 
%         Dance \\
%         DBLP-Google Scholar &
%         Citation & 
%         4 & 
%         5,347 & 
%         66,879 & 
%         Venue & 
%         VLDB J \\
%         DBLP-ACM &
%         Citation & 
%         4 & 
%         2,220 & 
%         4,910 & 
%         Authors & 
%         Female \\
%         Febrl &
%         Patients & 
%         7 & 
%         8,520 & 
%         12,983 & 
%         Given\_Name & 
%         Female \\
%     \bottomrule
%     \end{tabular}
%     \caption{Datasets, their domains, characteristics, and sensitive attributes with values.}
%     \vspace{-2mm}
%     \label{tab:datasets}
% \end{table*}
% }



% \begin{table*}[htbp]
% \centering
% \footnotesize
% \begin{tabularx}{0.902\textwidth}{|l|l|c|c|c|c|c|}
% \hline
% \textbf{Dataset} & \textbf{Domain} & \textbf{\# Attributes} & \textbf{\# Matching Pairs} & \textbf{Total Records} & \textbf{Sensitive Attribute} & \textbf{Sensitive Value} \\ \hline
% Walmart-Amazon   & Electronics      & 5                      & 962                        & 24,628                 & Category                     & Printers \\ \hline
% Beer             & Beer             & 4                      & 68                         & 7,345                  & Beer\_Name                   & Red      \\ \hline
% Amazon-Google    & Software         & 3                      & 1,167                      & 4,589                  & Manufacturer                 & Microsoft \\ \hline
% Fodors-Zagat     & Restaurant       & 6                      & 110                        & 864                    & Type                         & Asian    \\ \hline
% iTunes-Amazon    & Music            & 8                      & 132                        & 62,830                 & Genre                        & Dance    \\ \hline
% DBLP-Google Scholar & Citation      & 4                      & 5,347                      & 66,879                 & Venue                        & VLDB J   \\ \hline
% DBLP-ACM         & Citation         & 4                      & 2,220                      & 4,910                  & Authors                      & Female   \\ \hline
% Febrl            & Patients         & 7                      & 8,520                      & 12,983                 & Given\_Name                  & Female   \\ \hline
% \end{tabularx}
% \caption{Datasets, their domains, characteristics, and sensitive attributes with values.}
% \label{tab:datasets}
% \end{table*}


% \begin{enumerate}[a)]
%     \item \textit{Standard Blocking}~\cite{fellegi1969theory}: This hash-based method groups records using concatenated attribute values (blocking keys) to form redundancy-free blocks. However, it is sensitive to noise; any variation in the key may exclude matching records from the same block.

%     \item \textit{Q-Grams and Extended Q-Grams Blocking}: Q-grams blocking splits blocking keys into subsequences of \textit{q} characters, improving noise tolerance but potentially increasing block size and number. Extended Q-Grams further combines q-grams for more distinctive keys, reducing block size and enhancing efficiency~\cite{christen2011survey, papadakis2015schema}.

%     \item \textit{Suffix and Extended Suffix Arrays Blocking}: Suffix Arrays Blocking converts blocking keys into suffixes of a minimum length to form blocks, filtering out common suffixes to prevent oversized blocks. Extended Suffix Arrays consider all substrings longer than the minimum length, boosting noise tolerance~\cite{christen2011survey, papadakis2015schema}.

%     \item \textit{AutoEncoder (\AutoBlcok) and Cross-Tuple Training (\CTT) Blocking}: These deep learning methods group similar records into blocks using embeddings. \AutoBlcok generates embeddings via an autoencoder to handle diverse and noisy data, while \CTT uses a Siamese Summarizer to create embeddings from synthetic data, enhancing distinction between matching and non-matching tuples~\cite{mudgal2018deep}.
% \end{enumerate}



% \starter{Blocking Methods} This section summarizes the blocking methods used in our study, encompassing both traditional and deep learning-based approaches.

% \textit{Standard Blocking}~\cite{fellegi1969theory}: A hash-based method groups records into blocks using concatenated attribute values (blocking keys). This approach creates redundancy-free blocks of entities with identical keys but is highly sensitive to noise, as variations in the blocking key can cause matching records to be excluded from the same block


% \textit{Q-Grams and Extended Q-Grams Blocking}~\cite{christen2011survey, papadakis2015schema}: Q-grams blocking enhances Standard Blocking by breaking down blocking keys into subsequences of q characters, creating more noise-tolerant blocks. However, it can lead to larger and more numerous blocks. Extended Q-Grams Blocking refines this by combining q-grams to create more distinctive blocking keys, reducing block size and count, thus improving efficiency and effectiveness.



% \textit{Suffix and Extended Suffix Arrays Blocking}~\cite{christen2011survey, papadakis2015schema}: Suffix Arrays Blocking overcomes some limitations of Standard Blocking by converting blocking keys into suffixes of a specified minimum length, forming blocks based on these suffixes and filtering out high-frequency ones to avoid large, unnecessary blocks. Extended Suffix Arrays Blocking further enhances this approach by considering all substrings longer than the minimum length, improving noise tolerance, especially at the end of blocking keys.


% \textit{AutoEncoder (\AutoBlcok) and Cross-Tuple Training (\CTT) Blocking}~\cite{mudgal2018deep}: These methods are deep learning-based approaches designed to optimize record matching by efficiently grouping similar records into blocks, thereby reducing the number of pairwise comparisons. \AutoBlcok uses an autoencoder to generate fixed-size embeddings from variable-length word sequences, capturing essential features in a dense, lower-dimensional space while minimizing reconstruction loss, which helps handle diverse and noisy datasets. Conversely, \CTT Blocking employs a Siamese Summarizer to create embeddings from synthetic training data, enhancing the distinction between matching and non-matching tuples by maximizing the similarity of matching pairs and minimizing it for non-matching ones. Both methods effectively facilitate blocking by utilizing these embeddings to group similar tuples, ensuring that only the most relevant pairs are considered during the matching process.

% This section provides an overview of the blocking methods employed in our study, which include both traditional and deep learning-based approaches. These methods are carefully selected to optimize the balance between computational efficiency and accuracy in EM tasks. By leveraging a variety of techniques, we aim to evaluate the effectiveness of each method in handling diverse datasets and maintaining fairness across different demographic groups.
% \mhm{checked until here}

% a basic hash-based method that groups records into blocks based on the concatenation of selected attribute values (blocking keys). The method forms blocks of entities with identical keys, leading to redundancy-free blocks. However, it is highly sensitive to noise, as any variation in the blocking key can lead to the exclusion of matching records from the same block.

% Q-grams blocking improves upon Standard Blocking by converting blocking keys into subsequences of q characters (q-grams). Each q-gram forms a block, making the method more resilient to noise. However, it may result in larger and more blocks compared to Standard Blocking.   Extended Q-Grams Blocking refines the Q-Grams method by using combinations of q-grams, which are concatenated to form more distinctive blocking keys. This approach reduces the number and size of blocks, improving the method's efficiency and effectiveness.

% Suffix Arrays Blocking addresses some of the limitations of Standard Blocking by converting blocking keys into suffixes longer than a predetermined minimum length. It creates blocks based on these suffixes, filtering out high-frequency suffixes to avoid large, unnecessary blocks.Extended Suffix Arrays Blocking further improves upon SA by considering not just suffixes but all substrings of blocking keys longer than a minimum length. This makes the method more effective in handling noise, particularly at the end of blocking keys.



 


% \textit{AutoEncoder DeepBlocker}~\cite{mudgal2018deep} is a deep learning-based method that employs an autoencoder model to generate fixed-size embeddings from variable-length word sequences in tuples. The autoencoder compresses the input sequences into a dense, lower-dimensional space that captures the most important features of the data. These embeddings are then used to group similar records into blocks, effectively reducing the number of pairwise comparisons needed in the matching process. By minimizing the reconstruction loss during training, the autoencoder ensures that the generated embeddings retain crucial information, making this method particularly effective in handling diverse and noisy datasets.

% \textit{Cross-Tuple Training (CTT) Blocking}~\cite{mudgal2018deep} is a deep learning approach that focuses on creating synthetic training data by modifying tuples to generate both matching and non-matching pairs. This method utilizes a Siamese Summarizer to produce embeddings that maximize the similarity between matching tuples while minimizing the similarity between non-matching ones. These embeddings are used to perform blocking by grouping similar tuples into blocks, ensuring that only the most relevant pairs are compared in the matching stage.

\ignore{\begin{table}[h!]
    \centering
    \small
    \resizebox{0.49\textwidth}{!}{
    \begin{tabular}{l c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c}
    \toprule
    Dataset & \multicolumn{3}{c}{\stdBlock} & \multicolumn{3}{c}{\exQgram} & \multicolumn{3}{c}{\exSuffix} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
     & \RR & \PC & \PQ & \RR & \PC & \PQ & \RR & \PC & \PQ \\
    \midrule
    \amzgog  & 99.73 & 98.29 & 9.58  & 99.70 & 94.17 & 8.41  & 99.86 & 83.89 & 15.85 \\
    \walamz  & 99.81 & 99.06 & 0.90  & 99.75 & 98.75 & 0.69  & 99.97 & 88.46 & 4.31  \\
    \DBLPGogS & 99.94 & 98.73 & 5.34  & 99.95 & 97.59 & 5.99  & 99.99 & 76.55 & 17.80 \\
    \DBLPACM & 99.94 & 99.86 & 66.26 & 99.94 & 99.96 & 60.25 & 99.94 & 99.46 & 60.33 \\
    \Beer    & 99.91 & 95.59 & 0.54  & 99.90 & 91.18 & 0.48  & 99.95 & 89.71 & 0.89  \\
    \FodorZag & 98.72 & 99.10 & 4.88  & 98.88 & 99.10 & 5.56  & 99.33 & 96.40 & 9.04  \\
    \itunamz & 99.86 & 96.97 & 0.02  & 99.77 & 71.21 & 0.01  & 99.99 & 51.52 & 0.19  \\
    \Febrl   & 99.87 & 70.96 & 10.78 & 99.93 & 65.54 & 18.60 & 99.95 & 59.46 & 26.40 \\
    \bottomrule
    \end{tabular}
    }
    \caption{\RR, \PC, and \PQ for traditional models across datasets.}
    \label{tab:transposed_tmp}    
\end{table}}





\begin{table*}[h!]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c}
    \toprule
    \multirow{2}{*}{Model} & \multicolumn{3}{c}{\amzgog} & \multicolumn{3}{c}{\walamz} & \multicolumn{3}{c}{\DBLPGogS} & \multicolumn{3}{c}{\DBLPACM} & \multicolumn{3}{c}{\Beer} & \multicolumn{3}{c}{\FodorZag} & \multicolumn{3}{c}{\itunamz} & \multicolumn{3}{c}{\Febrl}\\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19} \cmidrule(lr){20-22} \cmidrule(lr){23-25}
     & \RR & \PC & \PQ & \RR & \PC & \PQ & \RR & \PC & \PQ & \RR & \PC & \PQ & \RR & \PC & \PQ & \RR & \PC & \PQ & \RR & \PC & \PQ & \RR & \PC & \PQ \\
    \midrule
    \stdBlock  & \textbf{99.88} & \underline{94.00} & \textbf{21.65} & 99.76 & \textbf{99.38} & 0.71 & 99.88 & \underline{99.66} & 2.59 & \textbf{99.95} & \textbf{99.91} & \textbf{77.55} & \textbf{99.95} & \textbf{94.12} & \textbf{0.96} & \underline{99.34} & \textbf{100.0} & \underline{9.47} & \underline{99.88} & \textbf{93.94} & 0.03 & \underline{99.95} & 67.88 & 27.61\\
    
    \qgram  & 99.83 & \textbf{94.77} & 14.73 & 99.61 & \underline{98.75} & 0.43 & 99.59 & \textbf{99.83} & 0.77 & \textbf{99.95} & \textbf{99.91} & 67.52 & \underline{99.94} & \underline{91.18} & 0.75 & 99.32 & \textbf{100.0} & 9.16 & 99.78 & 78.03 & 0.01 & \underline{99.95} & 70.32 & \underline{30.97}\\
    
    \exQgram  & 99.82 & 93.40 & 13.91 & 99.53 & 96.05 & 0.35 & 99.57 & 99.57 & 0.74 & \textbf{99.95} & \textbf{99.91} & 71.92 & 99.93 & 89.71 & 0.70 & 99.33 & \underline{99.09} & 9.19 & 99.75 & 75.0 & 0.01 & \underline{99.95} & 64.61 & 28.11\\
    
    \suffix & \underline{99.87} & 89.20 & \underline{18.38} & \textbf{99.93} & 92.83 & \textbf{2.21} & \textbf{99.96} & 87.71 & \textbf{6.38} & \textbf{99.95} & \underline{99.86} & \underline{74.42} & \textbf{99.95} & \underline{91.18} & \textbf{0.96} & \textbf{99.35} & \textbf{100.0} & \textbf{9.60} & \textbf{99.99} & 55.3 & \textbf{0.21} & \textbf{99.96} & 60.82 & \textbf{32.06}\\
    
    \exSuffix & 99.86 & 84.06 & 16.38 & \underline{99.89} & 95.43 & \underline{1.52} & \underline{99.95} & 83.92 & \underline{4.94} & \underline{99.94} & 99.55 & 60.98 & \textbf{99.95} & 85.29 & \underline{0.85} & 99.26 & 96.36 & 8.14 & \textbf{99.99} & 51.52 & \underline{0.14} & \underline{99.95} & 62.79 & 28.07\\
    
    \AutoBlock & 98.45 & 76.26 & 1.31 & 99.77 & 82.74 & 0.62 & 99.92 & 82.06 & 3.35 & 97.82 & 97.61 & 1.66 & 98.33 & 85.29 & 0.03 & 84.89 & \textbf{100.0} & 0.41 & 99.91 & 80.30 & 0.03 & 99.23 & \underline{85.19} & 2.24\\
    
    \CTT & 98.45 & 85.26 & 1.46 & 99.77 & 90.75 & 0.68 & 99.92 & 89.55 & 3.66 & 97.82 & 99.23 & 1.68 & 98.33 & 86.76 & 0.03 & 84.89 & \textbf{100.0} & 0.41 & 99.91 & \underline{81.82} & 0.03 & 99.23 & \textbf{90.86} & 2.39\\
    \bottomrule
    \end{tabular}
    }
    \caption{\RR, \PC, and \PQ for different models across datasets}
    \label{tab:position_prediction_metrics}    
\end{table*}


\begin{table*}[h!]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c}
    \toprule
    \multirow{2}{*}{Model} & \multicolumn{3}{c}{\amzgog} & \multicolumn{3}{c}{\walamz} & \multicolumn{3}{c}{\DBLPGogS} & \multicolumn{3}{c}{\DBLPACM} & \multicolumn{3}{c}{\Beer} & \multicolumn{3}{c}{\FodorZag} & \multicolumn{3}{c}{\itunamz} & \multicolumn{3}{c}{\Febrl}\\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19} \cmidrule(lr){20-22} \cmidrule(lr){23-25}
     & \RR & \PC & \PQ & \RR & \PC & \PQ & \RR & \PC & \PQ & \RR & \PC & \PQ & \RR & \PC & \PQ & \RR & \PC & \PQ & \RR & \PC & \PQ & \RR & \PC & \PQ \\
    \midrule
    \stdBlock  & 0.03 & 5.98 & 7.87 & 0.21 & \textbf{0.57} & \underline{0.07} & \textbf{0.00} & \underline{0.18} & \textbf{0.10} & \textbf{0.01} & \textbf{0.10} & 9.15 & \underline{0.02} & 4.24 & 0.07 & 0.28 & \textbf{0.00} & \textbf{0.04} & 0.11 & \underline{2.07} & 0.02 & \textbf{0.02} & 1.82 & 11.66\\
    
    \qgram  & 0.20 & \textbf{1.52} & 10.45 & 1.26 & 1.37 & 0.26 & 0.09 & \textbf{0.09} & 0.18 & \underline{0.02} & \textbf{0.10} & 1.98 & \textbf{0.01} & 9.37 & \underline{0.02} & \underline{0.23} & \textbf{0.00} & 0.92 & 0.17 & 10.00 & \underline{0.01} & \textbf{0.02} & 1.01 & 11.09\\
    
    \exQgram  & 0.27 & \underline{1.68} & 10.69 & 0.52 & \underline{0.59} & \textbf{0.01} & 0.09 & 0.19 & \underline{0.16} & \textbf{0.01} & \textbf{0.10} & 7.20 & \textbf{0.01} & 5.92 & 0.07 & \textbf{0.22} & \underline{1.00} & 1.10 & 0.18 & 7.17 & \textbf{0.00} & \textbf{0.02} & 1.55 & 9.79\\
    
    \suffix & \underline{0.01} & 18.48 & 7.73 & \textbf{0.01} & 2.11 & 3.58 & \underline{0.01} & 0.68 & 1.30 & \textbf{0.01} & \underline{0.16} & 7.95 & \underline{0.02} & 3.36 & 0.04 & 0.15 & \textbf{0.00} & 2.28 & \textbf{0.00} & \textbf{0.43} & 0.04 & \textbf{0.02} & 1.39 & 12.49\\
    
    \exSuffix & \underline{0.01} & 20.09 & 7.63 & \underline{0.03} & 2.47 & 2.45 & 0.02 & 1.66 & 1.20 & \textbf{0.01} & 0.52 & 9.42 & \underline{0.02} & 7.61 & 0.08 & 0.19 & 4.00 & 1.45 & \textbf{0.00} & 2.17 & 0.06 & \textbf{0.02} & 1.21 & 11.58\\
    
    \AutoBlock & \textbf{0.00} & 10.11 & \underline{0.39} & \textbf{0.01} & 13.53 & 0.40 & \textbf{0.00} & 3.83 & 0.27 & 0.21 & 2.02 & \underline{0.33} & 0.11 & \underline{1.59} & \textbf{0.01} & 0.45 & \textbf{0.00} & \underline{0.18} & \underline{0.04} & 11.20 & \underline{0.01} & 0.11 & \underline{0.54} & \textbf{1.47}\\
    
    \CTT & \textbf{0.00} & 2.04 & \textbf{0.29} & \textbf{0.01} & 12.33 & 0.59 & \underline{0.01} & 1.92 & 0.67 & 0.26 & 0.89 & \textbf{0.32} & 0.07 & \textbf{0.97} & \textbf{0.01} & 1.30 & \textbf{0.00} & 0.20 & \underline{0.04} & 6.20 & \textbf{0.00} & \underline{0.05} & \textbf{0.40} & \underline{1.74}\\
    \bottomrule
    \end{tabular}
    }
    \caption{\RR, \PC, and \PQ  disparities for different models across datasets}
    \label{tab:position_prediction_metrics2}    
\end{table*}





\begin{table*}[h!]
    \centering
    \tiny
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c}
    \toprule
    \multirow{2}{*}{Model} 
    & \multicolumn{6}{c}{\walamz} 
    & \multicolumn{6}{c}{\DBLPGogS} 
    & \multicolumn{6}{c}{\DBLPACM} 
    & \multicolumn{6}{c}{\Beer} \\
    
    \cmidrule(lr){2-7} \cmidrule(lr){8-13} \cmidrule(lr){14-19} \cmidrule(lr){20-25}
     & $\RR_1$ & $\RR_2$ & $\PC_1$ & $\PC_2$ & $\PQ_1$ & $\PQ_2$ 
     & $\RR_1$ & $\RR_2$ & $\PC_1$ & $\PC_2$ &$\PQ_1$ & $\PQ_2$ 
     & $\RR_1$ & $\RR_2$ & $\PC_1$ & $\PC_2$ & $\PQ_1$ & $\PQ_2$ 
     & $\RR_1$ & $\RR_2$ & $\PC_1$ & $\PC_2$ & $\PQ_1$ & $\PQ_2$ \\


     
    \midrule
    \stdBlock  
    & 99.88 & 99.93 & 97.73 & 97.83 & 2.76 & 2.40 
    & 99.99 & 99.99 & 96.28 & 97.35 & 43.84 & 38.21 
    & 99.96 & 99.95 & 100.0 & 99.90 & 69.82 & 78.97 
    & 99.96 & 99.94 & 96.55 & 92.31 & 0.92 & 0.99 \\
    
    \qgram  
    & 99.66 & 99.89 & 96.59 & 97.83 & 0.99 & 1.47 
    & 99.99 & 99.98 & 96.03 & 98.12 & 35.18 & 19.04 
    & 99.96 & 99.94 & 100.0 & 99.90 & 65.82 & 67.80 
    & 99.94 & 99.93 & 96.55 & 87.18 & 0.74 & 0.76 \\
    
    \exQgram  
    & 99.72 & 99.82 & 96.59 & 95.65 & 1.18 & 0.86 
    & 99.99 & 99.98 & 95.78 & 96.24 & 33.39 & 18.87 
    & 99.96 & 99.95 & 100.0 & 99.90 & 65.82 & 73.02 
    & 99.94 & 99.93 & 93.1  & 87.18 & 0.66 & 0.73 \\
    
    \suffix 
    & 99.97 & 99.96 & 88.64 & 91.08 & 9.51 & 3.44 
    & 99.99 & 99.99 & 83.13 & 83.43 & 16.92 & 18.34 
    & 99.96 & 99.95 & 100.0 & 99.84 & 67.69 & 75.64 
    & 99.96 & 99.94 & 93.1  & 89.74 & 0.98 & 0.94 \\
    
    \exSuffix 
    & 99.97 & 99.96 & 87.5  & 88.79 & 10.25 & 4.11 
    & 99.99 & 99.99 & 75.19 & 77.83 & 16.14 & 18.55 
    & 99.95 & 99.94 & 100.0 & 99.48 & 53.08 & 62.50 
    & 99.96 & 99.94 & 89.66 & 82.05 & 0.90 & 0.82 \\
    
    \AutoBlock 
    & 99.78 & 99.77 & 92.05 & 96.80 & 1.47 & 0.69 
    & 99.91 & 99.92 & 95.53 & 94.90 & 3.12 & 3.96 
    & 98.18 & 97.74 & 100.0 & 99.84 & 1.54 & 1.72 
    & 98.29 & 98.38 & 86.21 & 84.62 & 0.02 & 0.03 \\
    
    \CTT 
    & 99.77 & 99.77 & 93.18 & 97.94 & 1.37 & 0.70 
    & 99.92 & 99.92 & 95.53 & 95.77 & 3.43 & 3.96 
    & 97.99 & 97.78 & 100.0 & 99.84 & 1.39 & 1.76 
    & 98.38 & 98.29 & 96.55 & 92.31 & 0.03 & 0.03 \\
    \bottomrule
    \end{tabular}
    }
    \caption{$RR_{1}$ is minority and the other majority}
    \label{tab:position_prediction_metrics2}    
\end{table*}



besides those measures that take into account the effectiveness of blocking methods, also the efficiney of them is also important, in other words run time of blokcing method play a cruitioal role on selecting the optimal blocking method, becuase if we meglect this factor, one can use a matching technique, which will result in a hich \RR, \PC, and \PQ but it will probably takes days to run. 

In contrast with accuracy measures in ML, there is not a much an agreement in blockinh measures in the literature, some works only consider \PC and \RR ~\cite{zhang2020autoblock,thirumuruganathan2021deep,ebraheem2017deeper,papadakis2011efficient,paulsen2023sparkly,papadakis2012blocking,michelson2006learning,bilenko2006adaptive,steorts2014comparison}. some others only used \PC and runtime ~\cite{galhotra2021efficient,li2018matchcatcher,zeakis2023pre,sarma2011cblock}. there was aslso some research that people used \textit{harmonic mean} between two measures which is defined as $ F_{a,b} = \frac{2 \times a \times b}{a+b}$ as the harmonic mean of $a$ and $b$. there is not also an agreement to use the harmonic mean between whcich measures. ~\cite{o2019review,o2018new,kopcke2010frameworks,kejriwal2013unsupervised,mugeni2023graph,mugeni2023graph} used the harmonic mean of \PC and \RR  while ~\cite{christen2011survey} used harmonic mean of \PC and \PQ. some also only considered \PC and \PQ ~\cite{javdani2019deepblock, de2009robust}.

this work tried to combine time and harmonic mean to have a single blocking measure, but they did that in not a correct way. they defined runtime as the time needed for doing blocking and matching part combined, and they calculated the harmonic mean of precision and recall at the end of EM pipeline. they used $\sqrt{time^2 + (1- F_{precision,recall})^2}$ as evaulation metric and tried to minimize that, but due to the fact that time is differenct of harmonic mean by nature it is not a correct way of combining these metrics together. 

There is no proper explanation on whcich blocking measures are more important and what is the relation of them with each other. ~\cite{papadakis2016comparative, zeakis2023pre, papadakis2011efficient,kejriwal2013unsupervised} very briefly touched this area and their explanation was that \PQ in blocking method is usually low, because if we were able to have high \PC and \PQ there is no need for a further matching and achiving a high \PQ is the task that matcher do. However, this explanation is not enough. In this study we calim that having only \PC, \RR, and runtime is enough for measugin the effectiveness of different blocking method and \PQ is related to \PC and \RR. Datasets that are used for blocking have a large number of pairs (order of millions) otherwise there is no need for blocking, and number of true matchs is usually in the order of thousands. For a good blkcing method \RR is above $90\%$ (usually $\approx99\%$) and as a result \PQ for a \PC of 1 can be only $10\%$, and a very small change in the \RR (in the order of $0.01\%$ in most dataset can have a huge effect on the candidate set size and this change will cause \PQ to be very sensistive. This is one of the reasons that only \PC, \RR, and runtime are needed. Also, due to the usuall size of \candidatePairs, \pairs, and \equivPairs that we discussed, \PQ have correlation with the combination if \RR and \PC and one can only focus on this two metric. Also, \PC and \RR has a trade-off, maximizing only one can lead to a decrease of other, for this reason similar to earlier works that we mentioned, we also use the harminic mean of \PC and \RR as follows: 



\begin{align}
F_B= \frac{2 \times \PC \times \RR}{\PC + \RR}
\end{align}





\begin{figure}
         \centering
        \subfloat[correlation matrix]{\label{fig:correlation_heatmap}
			{\includegraphics[width=0.23\textwidth]{figs/correlation_heatmap_all.pdf}}}	
         \subfloat[later]{\label{fig:later}
			{\includegraphics[width=0.23\textwidth]{figs/later.pdf}}}

 \caption{Fig. ~\ref{fig:correlation_heatmap} displays the correlation of various blocking measures.}\label{fig:exp1}
\end{figure}





\begin{table*}[h!]
    \centering
    \small
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in} c@{\hskip 0.05in} c@{\hskip 0.05in} c@{\hskip 0.05in}}
    \toprule
    \multirow{2}{*}{Model} & \multicolumn{4}{c}{\amzgog} & \multicolumn{4}{c}{\walamz} & \multicolumn{4}{c}{\DBLPGogS} & \multicolumn{4}{c}{\DBLPACM} & \multicolumn{4}{c}{\Beer} & \multicolumn{4}{c}{\FodorZag} & \multicolumn{4}{c}{\itunamz} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17} \cmidrule(lr){18-21} \cmidrule(lr){22-25} \cmidrule(lr){26-29}
     & \RR & \PC & \PQ & \Fb & \RR & \PC & \PQ & \Fb & \RR & \PC & \PQ & \Fb & \RR & \PC & \PQ & \Fb & \RR & \PC & \PQ & \Fb & \RR & \PC & \PQ & \Fb & \RR & \PC & \PQ & \Fb \\
    \midrule
\stdBlock & 
99.73 & 98.29 & 9.58 & 99.00 & 
99.81 & 99.06 & 0.90 & 99.44 & 
99.94 & 98.73 & 5.34 & 99.33 & 
99.94 & 99.86 & 66.26 & 99.90 & 
99.91 & 95.59 & 0.54 & 97.70 & 
98.72 & 99.10 & 4.88 & 98.91 & 
99.86 & 97.73 & 0.02 & 98.78 \\

\qgram & 
99.69 & 95.72 & 8.29 & 97.66 & 
99.77 & 99.06 & 0.75 & 99.42 & 
99.95 & 98.75 & 6.22 & 99.34 & 
99.94 & 99.95 & 59.22 & 99.95 & 
99.90 & 92.65 & 0.51 & 96.14 & 
98.83 & 99.10 & 5.31 & 98.96 & 
99.79 & 73.48 & 0.01 & 84.64 \\

\exQgram & 
99.70 & 94.17 & 8.40 & 96.86 & 
99.75 & 98.75 & 0.69 & 99.25 & 
99.95 & 97.59 & 5.99 & 98.75 & 
99.94 & 99.95 & 60.25 & 99.95 & 
99.90 & 91.18 & 0.48 & 95.34 & 
98.88 & 99.10 & 5.56 & 98.99 & 
99.77 & 71.97 & 0.01 & 83.62 \\

\suffix & 
99.85 & 88.52 & 16.06 & 93.84 & 
99.96 & 91.16 & 3.49 & 95.36 & 
99.98 & 82.38 & 16.61 & 90.33 & 
99.95 & 99.91 & 73.06 & 99.93 & 
99.95 & 88.24 & 0.88 & 93.73 & 
99.31 & 99.10 & 9.03 & 99.20 & 
99.99 & 50.76 & 0.24 & 67.34 \\

\exSuffix & 
99.86 & 83.89 & 15.85 & 91.18 & 
99.97 & 88.36 & 4.31 & 93.80 & 
99.99 & 76.47 & 17.78 & 86.66 & 
99.94 & 99.46 & 60.34 & 99.70 & 
99.95 & 89.71 & 0.89 & 94.55 & 
99.33 & 96.40 & 9.04 & 97.84 & 
99.99 & 51.52 & 0.19 & 68.00 \\

\AutoBlock & 
98.45 & 88.52 & 1.52 & 93.22 & 
99.77 & 96.36 & 0.73 & 98.04 & 
99.92 & 95.23 & 3.89 & 97.52 & 
97.82 & 99.86 & 1.69 & 98.83 & 
98.33 & 85.29 & 0.03 & 91.35 & 
84.89 & 99.10 & 0.41 & 91.45 & 
99.91 & 90.15 & 0.03 & 94.78 \\

\CTT & 
98.45 & 95.97 & 1.64 & 97.20 & 
99.77 & 97.51 & 0.73 & 98.63 & 
99.92 & 95.96 & 3.92 & 97.90 & 
97.82 & 99.86 & 1.69 & 98.83 & 
98.33 & 94.12 & 0.03 & 96.18 & 
84.89 & 99.10 & 0.41 & 91.45 & 
99.91 & 91.67 & 0.04 & 95.61 \\


\graphblk & 
 97.74 & 93.92 & 1.10 & 95.78 & 
97.59 & 83.89 & 0.06 & 90.22 & 
98.14 & 79.13 & 0.14 & 87.61 &
99.96 & 98.78 & 82.79 & 99.37 &
 98.91 & 88.24 & 0.04 & 93.27 & 
 80.17 & 20.54 & 0.07 & 32.70 & 
98.37 & 54.55 & 0.001 & 70.18 \\


    \bottomrule
    \end{tabular}
    }
    \caption{\Fb disparities and \Fb values within the minority and majority groups}
    \label{tab:delta-fb}    
\end{table*}







\begin{table*}[h!]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c}
    \toprule
    \multirow{2}{*}{Model} & \multicolumn{3}{c}{\amzgog} & \multicolumn{3}{c}{\walamz} & \multicolumn{3}{c}{\DBLPGogS} & \multicolumn{3}{c}{\DBLPACM} & \multicolumn{3}{c}{\Beer} & \multicolumn{3}{c}{\FodorZag} & \multicolumn{3}{c}{\itunamz}\\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19} \cmidrule(lr){20-22} 
     & $\Delta\RR$ & $\Delta\PC$ & $\Delta F_{B}$ & $\Delta\RR$ & $\Delta\PC$ & $\Delta F_{B}$ & $\Delta\RR$ & $\Delta\PC$ & $\Delta F_{B}$ & $\Delta\RR$ & $\Delta\PC$ & $\Delta F_{B}$ & $\Delta\RR$ & $\Delta\PC$ & $\Delta F_{B}$ & $\Delta\RR$ & $\Delta\PC$ & $\Delta F_{B}$ & $\Delta\RR$ & $\Delta\PC$ & $\Delta F_{B}$\\
    \midrule
\stdBlock & 
0.08 & 1.71 & 0.91 & 
0.14 & 1.47 & 0.81 & 
-0.05 & 0.77 & 0.37 & 
-0.01 & -0.16 & -0.08 & 
-0.01 & -1.68 & -0.88 & 
0.01 & -0.99 & -0.49 & 
-0.13 & 7.50 & 3.83 \\

\qgram & 
0.38 & -1.00 & -0.33 & 
0.25 & 1.47 & 0.87 & 
-0.03 & 1.33 & 0.66 & 
-0.01 & -0.05 & -0.03 & 
-0.01 & -6.81 & -3.65 & 
-0.20 & -0.99 & -0.59 & 
-0.15 & -9.35 & -6.13 \\

\exQgram & 
0.41 & 6.16 & 3.53 & 
0.18 & 1.13 & 0.66 & 
-0.03 & 1.15 & 0.58 & 
-0.01 & -0.05 & -0.03 & 
-0.01 & -9.37 & -5.09 & 
-0.16 & -0.99 & -0.57 & 
-0.20 & -0.76 & -0.58 \\

\suffix & 
0.07 & 16.01 & 9.77 & 
-0.01 & 5.28 & 2.95 & 
-0.00 & 0.27 & 0.16 & 
-0.01 & -0.10 & -0.06 & 
-0.02 & -8.49 & -4.77 & 
-0.18 & -0.99 & -0.58 & 
-0.00 & 1.09 & 0.96 \\

\exSuffix & 
0.04 & 18.16 & 11.79 & 
-0.00 & 0.94 & 0.53 & 
0.00 & 1.66 & 1.07 & 
-0.01 & -0.63 & -0.32 & 
-0.02 & -5.92 & -3.28 & 
-0.18 & -3.96 & -2.09 & 
-0.00 & 2.17 & 1.90 \\

\AutoBlock & 
-0.01 & 8.98 & 5.20 & 
-0.01 & 4.75 & 2.50 & 
0.01 & -0.60 & -0.30 & 
-0.48 & -0.16 & -0.32 & 
0.04 & -1.59 & -0.89 & 
0.90 & -0.99 & 0.11 & 
-0.04 & -6.96 & -3.81 \\

\CTT & 
-0.01 & 2.78 & 1.44 & 
0.01 & 4.76 & 2.49 & 
0.01 & 0.46 & 0.24 & 
-0.21 & -0.16 & -0.18 & 
-0.09 & -4.24 & -2.25 & 
0.00 & -0.99 & -0.42 & 
-0.04 & -1.20 & -0.67 \\


\graphblk & 
0.30 & 2.37  & 1.39 & 
0.81 & 17.29  & 11.13 & 
1.39 & -7.28 & -3.70 & 
-0.01 & -1.04 & -0.53 & 
-0.24 & -2.48 & -1.49 & 
-2.99 & 11.78  & 16.37 & 
-1.09& -4.24& -3.76  \\






    
    \bottomrule
    \end{tabular}
    }
    \caption{\RR, \PC, and \Fb  disparities for different models across datasets: Major - Minor}
    \label{tab:position_prediction_metrics2}    
\end{table*}





\begin{table*}[h!]
    \centering
    \tiny
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c}
    \toprule
    \multirow{2}{*}{Model} 
    & \multicolumn{6}{c}{\amzgog} 
    & \multicolumn{6}{c}{\walamz} 
    & \multicolumn{6}{c}{\Beer} 
    & \multicolumn{6}{c}{\FodorZag} \\
    
    \cmidrule(lr){2-7} \cmidrule(lr){8-13} \cmidrule(lr){14-19} \cmidrule(lr){20-25}
     & $\RR_1$ & $\RR_2$ & $\PC_1$ & $\PC_2$ & $F_1$ & $F_2$ 
     & $\RR_1$ & $\RR_2$ & $\PC_1$ & $\PC_2$ &$F_1$ & $F_2$ 
     & $\RR_1$ & $\RR_2$ & $\PC_1$ & $\PC_2$ & $F_1$ & $F_2$ 
     & $\RR_1$ & $\RR_2$ & $\PC_1$ & $\PC_2$ & $F_1$ & $F_2$ \\

    \midrule
\stdBlock & 
99.66 & 99.73 & 96.67 & 98.37 & 98.14 &  99.05 & 
99.68 & 99.82 & 97.73 & 99.20 & 98.69 &  99.51 & 
99.91 & 99.90 & 96.55 & 94.87 & 98.20 &  97.32 & 
98.71 & 98.72 & 100.00 & 99.01 & 99.35 &  98.87 \\

\qgram & 
99.33 & 99.72 & 96.67 & 95.66 & 97.98 &  97.65 & 
99.54 & 99.79 & 97.73 & 99.20 & 98.62 &  99.49 & 
99.91 & 99.90 & 96.55 & 89.74 & 98.20 &  94.55 & 
99.00 & 98.80 & 100.00 & 99.01 & 99.50 &  98.90 \\

\exQgram & 
99.32 & 99.73 & 88.33 & 94.49 & 93.51 &  97.04 & 
99.58 & 99.76 & 97.73 & 98.86 & 98.65 &  99.31 & 
99.90 & 99.90 & 96.55 & 87.18 & 98.20 &  93.11 & 
99.01 & 98.86 & 100.00 & 99.01 & 99.50 &  98.93 \\

\suffix & 
99.79 & 99.86 & 73.33 & 89.34 & 84.54 &  94.31 & 
99.97 & 99.95 & 86.36 & 91.65 & 92.67 &  95.62 & 
99.96 & 99.94 & 93.10 & 84.62 & 96.41 &  91.64 & 
99.46 & 99.28 & 100.00 & 99.01 & 99.73 &  99.15 \\

\exSuffix & 
99.82 & 99.86 & 66.67 & 84.82 & 79.94 &  91.73 & 
99.97 & 99.96 & 87.50 & 88.44 & 93.32 &  93.85 & 
99.96 & 99.94 & 93.10 & 87.18 & 96.41 &  93.12 & 
99.48 & 99.30 & 100.00 & 96.04 & 99.74 &  97.64 \\

\AutoBlock & 
98.46 & 98.45 & 80.00 & 88.98 & 88.28 &  93.48 & 
99.79 & 99.77 & 92.05 & 96.80 & 95.76 &  98.26 & 
98.31 & 98.36 & 86.21 & 84.62 & 91.86 &  90.97 & 
84.12 & 85.02 & 100.00 & 99.01 & 91.38 &  91.49 \\

\CTT & 
98.46 & 98.45 & 93.33 & 96.12 & 95.83 &  97.27 & 
99.77 & 99.77 & 93.18 & 97.94 & 96.36 &  98.85 & 
98.38 & 98.29 & 96.55 & 92.31 & 97.46 &  95.20 & 
84.89 & 84.89 & 100.00 & 99.01 & 91.83 &  91.41 \\

\graphblk &
97.45 & 97.74 & 91.67 & 94.04 & 94.47 & 95.86 &
96.81 & 97.62 & 68.18 & 85.47 & 80.01 & 91.14 &
99.03 & 98.79 & 89.66 & 87.18 & 94.11 & 92.62 &
82.73 & 79.74 & 10.00 & 21.78 & 17.84 & 34.22 \\






    \bottomrule
    \end{tabular}
    }
    \caption{$RR_{1}$ is minority and the other majority}
    \label{tab:position_prediction_metrics2}    
\end{table*}



% \starter{Fairness in Entity Matching and Blocking} Fairness is a growing concern in EM systems, especially as they are used in data-driven decision-making. The main issue is that these systems can unintentionally reinforce biases in the data, resulting in unfair outcomes. This is particularly problematic in the blocking stage of EM, where the method of grouping records for comparison can introduce bias, impacting both accuracy and fairness in the matching process.

% Recent research has focused on addressing these fairness concerns in EM.~\cite{efthymiou2021fairer} introduced FairER, an algorithm designed to incorporate fairness constraints directly into the EM process. While FairER primarily addresses the matching phase, the principles it introduces are highly relevant to blocking as well. In blocking, the way records are grouped determines which pairs are compared, and biases in this stage can skew the entire matching process. By ensuring that different groups of entities, especially those belonging to protected categories, have similar chances of being accurately matched, FairER highlights the importance of fairness at the very beginning of the EM pipeline. This approach contrasts with traditional EM systems that prioritize accuracy without considering the potential for bias, which can be particularly problematic during the blocking stage if certain groups are underrepresented in blocks.

% A recent study ~\cite{shahbazi2024fairness} investigated fairness-aware data preparation techniques for EM, emphasizing the importance of addressing bias early in the process. This is particularly relevant to blocking methods, which must ensure that blocks are constructed without disproportionately excluding or grouping certain entities. Bias at this stage could lead to biased outcomes downstream, making it crucial to consider fairness to prevent systematic exclusion or misrepresentation of certain groups.

% Moreover, there is a growing interest in quantifying fairness in EM outcomes. ~\cite{nilforoushan2022entity} proposed an AUC-based fairness metric to evaluate the fairness of EM results. This metric provides a way to assess how well the EM system performs across different groups, offering insights into potential biases that may arise during the matching process. When applied to blocking, such metrics could be instrumental in evaluating and refining blocking methods to ensure they do not introduce or exacerbate biases.


% \mhm{I should fix below}

% \subsection{Fairness in Clustering} \label{sec:fair-cluster-rw}   Blocking can be seen as clustering entities before matching. We, therefore, briefly review fairness concepts in clustering as a related task. Fairness in clustering is assessed using metrics that ensure equitable treatment across demographic groups. In clustering, fairness is evaluated by the balance within clusters, using metrics like demographic parity and balance ratio~\cite{celis2023fairness} to measure proportional representation. Techniques such as {\em Fairlet Decomposition}~\cite{chhabra2021overview} utilize these metrics to create balanced groups across sensitive attributes before final clustering, ensuring fair representation. While having balanced clusters is a reasonable fairness requirement for clustering, it does not apply to blocking, where the goal is not equal representation within blocks but rather to create small blocks that include all equivalent record pairs.

%In ranking algorithms, fairness is measured by metrics assessing visibility and exposure across ranked lists. Fairness-Aware Ranking (FA*IR)~\cite{zehlike2020fair} and exposure fairness metrics, like those in FAIR-PG-RANK~\cite{singh2020fairpg}, aim to ensure balanced exposure for different groups, preventing systematic favoritism or marginalization.

%These fairness metrics are essential for developing unbiased algorithms and are crucial when designing metrics for fairness in blocking methods for entity matching. By ensuring equitable block formation, these metrics help identify and mitigate potential biases, promoting fairness throughout the entity matching process.


% Fairness in clustering and ranking algorithms is often assessed using specific metrics that ensure equitable treatment across different demographic groups. In clustering, fairness is typically evaluated by examining the balance within clusters. Metrics such as demographic parity and balance ratio~\cite{celis2023fairness} are used to measure the extent to which different groups are proportionately represented within each cluster. For instance, Fairlet Decomposition~\cite{chhabra2021overview} utilizes these metrics by forming small groups that are balanced across sensitive attributes before merging them into final clusters, thereby ensuring that no group is disproportionately represented or underrepresented in the clustering process.


% In ranking algorithms, fairness is commonly measured by metrics that assess the visibility and exposure of different groups across the ranked list. Fairness-Aware Ranking (FA*IR)~\cite{zehlike2020fair} uses a threshold-based metric to ensure that protected groups receive adequate visibility at different ranks, maintaining a balance between accuracy and fairness. Similarly, exposure fairness metrics, such as those used in FAIR-PG-RANK~\cite{singh2020fairpg}, evaluate how well the ranking process ensures equitable exposure for items representing different groups. These metrics focus on the distribution of ranks among different demographic groups, ensuring that no group is systematically favored or marginalized.

% These fairness metrics in clustering and ranking are crucial for developing equitable algorithms that do not propagate or exacerbate existing biases in data. Their relevance is particularly significant when designing metrics to measure fairness and bias in blocking methods for entity matching. In blocking, records are grouped together for comparison, similar to how items are clustered or ranked. To ensure fairness, it is essential to develop metrics that can evaluate whether the formation of blocks inadvertently favors or marginalizes certain groups. These metrics would enable a more precise evaluation of how equitable the blocking process is, helping to identify and mitigate any potential biases early in the entity matching pipeline. Consequently, such fairness-aware metrics are integral to promoting fairness and reducing bias in the overall entity matching process.




%These insights are invaluable for refining existing blocking methods and developing new techniques that aim to minimize these disparities. For instance, if a significant Pair Completeness Disparity is detected, the blocking criteria can be adjusted to ensure that minority groups are not disproportionately disadvantaged. Similarly, balancing the Reduction Ratio across groups can help ensure that the computational benefits of blocking are equitably distributed.

%The proposed method for quantifying biases in blocking techniques extends traditional performance metrics and introduces a critical framework for evaluating and improving the fairness of these methods.

% For $e_i$, there is a sensitive value $e_i.a$. $\mc{B}$ and $\mc{E}$....

% $E_i(x)$ the set of entities in dataset $\relation_i$ from group $x$, e.g., $E_1(a)$.

% $\mc{E}_a=\{(E_1(a)\times E_2) \cup (E_1\times E_2(a))\}$

% $\mc{E}_{a,\mc{B}}=\mc{E}_a\cap (\cup_{i\in [1,k]} \mc{B}_i)$


% $\RR_{a} = 1- \frac{E_1 \times E_2 - E_1(b) \times E_2(b)}{E_1 \times E_2}$

% $\RR_a=1-\frac{E_1(b)\times E_2(b)}{E_1\times E_2}$

% $\RR_b=\frac{E_1(a)\times E_2(a)}{E_1\times E_2}$

% $\trueMatch_a$

% In this section, we extend the quality metrics of blocking to assess bias in blocking techniques. To the best of our knowledge, no other studies have explored this aspect. For the same reason of EM process here we define a minoirty pair if at least one entity in that pair belongs to the minority group. we define three fairness metrics for blocking. RR disparity (\RRD), PC disparity (\PCD), and PQ disparity (\PQD). each one defines as difference of related metric between minority and majority group. 


% \(\text{RR}\xspace_{minority} = \) reduction of comparison space between pairs that at list one entity belongs to minority.

% \(\text{RR}\xspace_{majority} = \) reduction comparison space between pairs that both belongs to majority.


% \(\text{PC}\xspace_{majority} = \) ...

% \(\text{PC}\xspace_{majority} = \) ...



% \(\text{PQ}\xspace_{majority} = \) ...

% \(\text{PQ}\xspace_{majority} = \) ...




% \green{to be continued ...}



% \mostafa{Any ideas for removing biases in blocking should go here.}

% \mhm{we have to explore or invent sth, nothing yet}

==> foundations.tex <==
\section{Foundations} \label{sec:foundation}
%\fei{Continue point.}
We apply the concept of diversity constraints as proposed by Stoyanovich et. al~\cite{stoyanovich2018online} (Section~\ref{sec:set}).  We introduce a formal definition of these diversity constraints, study their validation, implication and satisfaction, define minimal cover, and present an axiomtization.  

%To capture diversity, we define a set of declarative \emph{diversity constraints} that specify lower and upper bounds on the number of attribute values in a relation. To express these constraints, we adopt the definition of diversity constraints in~\cite{stoyanovich2018online} that we reviewed in Section~\ref{sec:set}.  


\begin{definition} [Diversity Constraints] \label{df:div} A diversity constraint over a relation schema $\mc{R}$ is of the form $\sigma=(A[a], \lambda_l, \lambda_r)$ in which $A \in \mc{R}$, $a \in \nit{dom}(A)$ and $\lambda_l,\lambda_r$ are non-negative integers. The diversity constraint $\sigma$ is satisfied by a relation $R$ of schema $\mc{R}$ denoted $R \models \sigma$ if and only if there are at least $\lambda_l$ and at most $\lambda_r$ occurrences of the value $a$ in attribute $A$ of relation $R$. We call $[\lambda_l,\lambda_r]$ the frequency range and $A[a]$ the target value of $\sigma$. A set of diversity constraints $\Sigma$ is satisfied by $R$, denoted by $R\models \Sigma$, iff $R$ satisfies every $\sigma \in \Sigma$. \boxtheorem\end{definition}

\ignore{Following Definition~\ref{df:div}, \ignore{$(A[a], 0, \lambda_r)$ and $(A[a], \lambda_l, +\infty)$ are subsequently left-unbounded and right-unbounded diversity constraints with frequency ranges $[0,\lambda_r]$ and $[\lambda_l, +\infty)$.} we use $(A[a], \emptyset)$ to refer to a  diversity constraint with the empty frequency range. We call it a {\em false diversity constraint} since it is falsified by any relation with schema $\mc{R}$. Similarly, $(A[a], 0, +\infty)$ is a {\em true} diversity constraint that always holds.}

\subsection{Validation}\label{sec:validation}
The {\em validation problem} is to decide whether $R \models\sigma$. Assuming $\sigma=(A[a], \lambda_l, \lambda_r)$, we can run a query that counts the number of occurrences of the target value $a$ in attribute $A$ of $R$ and then check if this number lies in the frequency range $[\lambda_l, \lambda_r]$.
Diversity constraints can be extended to multiple attributes by replacing $A[a]$ with $X[t]$, where $X$ is a set of attributes and $t$ is a tuple with values from these attributes.  This extended diversity constraint $\sigma=(X[t], \lambda_l, \lambda_r)$ is satisfied by $R$ if there are at least $\lambda_l$ and at most $\lambda_r$ tuples in $R$ with the same attribute values in $t$. The validation problem for a multi-attribute diversity constraint is answered in a similar manner as the single attribute diversity constraint by extending the conditions to include each target attribute values, and aggregating the results via a count query.  Similar to traditional functional dependencies, validation is in PTIME since we can automatically generate SQL queries from the diversity constraints~\cite{FGJK08}.

%Note that the diversity constraints can be applied on any relation and are meaningful in general and independent of our application for representing diversity in data publishing in Section~\ref{sec:anon}. Our discussion about the validation problem in this section and the implication problem in Section~\ref{sec:implication} are about applying diversity constraints in general. 


\subsection{Implication and Axiomatization} \label{sec:implication}
We present an axiomatization for diversity constraints, \eat{that can be used to determine their implication.  We} and formally define the logical implication problem.
%Now we study the logical implication for diversity constraints and an axiomatization for testing it.

\begin{definition}[Logical Implication]
Given a set of diversity constraints $\Sigma$ over schema $\mc{R}$, and a diversity constraint $\sigma \not \in \Sigma$, we say $\Sigma$ {\em implies} $\sigma$, denoted by $\Sigma \models \sigma$, if and only if any relation $R \models \Sigma$, then $R \models \sigma$.  Given any finite set  $\Sigma$ and a constraint $\sigma$, the {\em implication problem} is to determine whether $\Sigma \models \sigma$.  
%If $\sigma$ is a logical implication of $\Sigma$, we also say $\Sigma$ implies or infers $\sigma$.
\boxtheorem\end{definition}

To test for logical implication $\Sigma \models \sigma$, and infer a new $\sigma$, we give a sound and complete axiomatization for diversity constraints.

%To test logical implication and infer new diversity constraints from a set of diversity constraints, we give an axiomatization with the following two axioms:

\starter{Axiom 1 (Fixed Attributes):} If $\sigma=(X[t],\lambda_l,\lambda_r)$, $\sigma'=(X[t],\lambda'_l,\lambda'_r)$, $[\lambda_l,\lambda_r] \subseteq [\lambda'_l,\lambda'_r]$, then $\sigma \models \sigma'$.

For example, let $\sigma'=(\att{GEN}[\val{Female}], 1, 5)$, and $\sigma=(\att{GEN}[\val{Female}],$ \ $ 2, 4)$, which require [1,5] and [2,4] females, respectively.  The frequency range of $\sigma'$ subsumes the range of $\sigma$, indicating that $\sigma$ is more restrictive.  Thus, if a relation $R$ satisfies $\sigma$, it also satisfies $\sigma'$.  
%that requires at leas $2$ and at most $4$ females in a relation. Both constraints are about the same target attribute value, i.e. the value \val{Female} for the attribute \att{GEN}. The difference is in their frequency ranges; the frequency range of $\sigma$ includes the frequency range of $\sigma'$. This means $\sigma'$ is a more restrictive version of $\sigma$. More precisely, if $\sigma'$ is satisfied by a relation, $\sigma$ is also satisfied by that relation. 


%\vspace{1mm}
%\noindent {\bf Axiom 2 (Fixed Ranges):} Let $\sigma=(X[t],\lambda_l,\lambda_r)$, $\sigma'=(X'[t'],\lambda_l,\lambda_r)$, $X\subseteq X'$ and $t \subseteq t'$, then $\sigma' \models \sigma$.

\starter{Axiom 2 (Attribute Extension):} Let $\sigma=(X[t], \lambda_l, \lambda_r)$, $\sigma'=(X'[t'], 0, \lambda_r)$, $X[t] \subset X'[t']$, then $\sigma \models \sigma'$.

Intuitively, if we add new target attribute values to a satisfied constraint, we cannot guarantee that there exist tuples with the added values ($\lambda_l' = 0$).  In contrast, if there exist tuples that contain the new target attribute values, their frequency would be upper bounded by $\lambda_r$. For example, if $\sigma=(\att{ETH}[ \val{Female}], 1,5)$ then we can infer $\sigma'=(\{\att{GEN},$ \ $ \att{ETH}\}[\val{Female},$ \ $ \val{Caucasian}], 0, 5)$. If there are between [1,5] females in $R$, we can infer at most $5$ are possibly Caucasian, but cannot state there is at least one Caucasian (i.e., the individuals may be of different ethnicity).
%\fei{The lower bound = 0 violates our defn of a diversity constraint in Sec. 3.1. This becomes an argument of the utility of a constraint with $\lambda_l$ = 0.  I changed the target values to avoid male-female only domain values as there are now other GENDER types :) Don't want to offend any reviewers.}

%\mostafa{I changed the definition. Neither $0$ nor $|R|$ were correct. The latter because we should not define the constraint for a particular relation. I changed the definition to be for schema $\mc{R}$ not a particular $R$.}
\eat{The description doesn't match the axiom, unless I am mis-understanding.  The description sounds like the implication is the other way around $\sigma \models \sigma'$.  Also, I thought the inference is on the lower bound, not the upper bound?  Our defn. of diversity constraints requires lower bound greater than 1.}

\starter{Axiom 3 (Attribute Reduction):} Let $\sigma=(X[t], \lambda_l, \lambda_r)$, $\sigma'=(X'[t'], \lambda_l, +\infty)$, $X'[t']\subset X[t]$, then $\sigma \models \sigma'$.

Axiom 3 states that for a satisfied diversity constraint $\sigma$, if we remove a set of target attribute values from $X[t]$, we can infer at least $\lambda_l$ occurrences of the values $X'[t'] \subset X[t]$.  For example, if $\sigma = (\{\att{GEN}, \att{ETH}\}[\val{Female}, \val{Caucasian}], 1,5)$ holds over $R$, then we can conclude at least $1$ individual is female, i.e., $\sigma' = (\att{ETH}[\val{Female}], 1, +\infty)$ holds.  However, we cannot claim the number of females in $R$ is limited to $5$ since there may be individuals from other ethnicities in $R$.
%since its target attribute values contain the one value in $\sigma$, i.e. \val{Female}, and has an additional attribute value, i.e. \val{Caucasian}.

\starter{Axiom 4 (Range Intersection):} Let $\sigma=(X[t],\lambda_l,\lambda_r)$, $\sigma'=(X[t]$\ $,\lambda'_l,\lambda'_r)$, then for any  $\sigma''=(X[t],\lambda''_l,\lambda''_r)$ where $[\lambda''_l,\lambda''_r] \subseteq [[\lambda_l,\lambda_r] $ \ $\cap [\lambda'_l,\lambda'_r]]$, it follows that $\{\sigma, \sigma'\} \models \sigma''$.

Intuitively, the set of tuples satisfying $\sigma, \sigma'$ would also satisfy a new diversity constraint $\sigma''$ that is more restrictive whose frequency range is the intersection of $[\lambda_l,\lambda_r]$ and $[\lambda'_l,\lambda'_r]$.  For example, let $\sigma=(\att{GEN}[\val{Female}], 1, 5)$ and $\sigma'=(\att{GEN}[\val{Female}], 3, 7)$, we can infer  $\sigma''=(\att{GEN}[\val{Female}], 3, 5)$.

\begin{theorem} The axiomatization (Ax. 1-4) is sound and complete.\end{theorem}

\emph{Proof Sketch.} Axioms 1-4 are sound as shown with the above examples. The axiomatization is also complete since any constraint $\sigma$ that can be inferred from $\Sigma$ can be obtained by applying Axioms 1-4 in a sequence.  We can prove this by showing for any $\sigma'$ that does not follow from $\Sigma$ via these axioms is not a logical implication of $\Sigma$, i.e., by construction of a relation that satisfies $\Sigma$ but not $\sigma'$.

We present Algorithm~\ref{alg:implies} that tests for logical implication by applying Axioms~1-4, i.e., checking whether $\Sigma \models \sigma$. The algorithm starts with a diversity constraint $(X[t], 0,+\infty)$ with the most general target range $\delta=[0,+\infty)$ (Line~\ref{ln:infty}), which is satisfied by any relation, hence, is inferred from $\Sigma$. The algorithm iterates over each constraint in $\Sigma$ to find constraints $\sigma'$ with target values in $\sigma$ to infer more restricted ranges $\delta$. Using Axioms~1-3 and in Lines~\ref{ln:intersect}-\ref{ln:left}, the algorithm subsequently finds target ranges $[\lambda'_l,\lambda'_r]$, $[0,\lambda'_r]$, and $[\lambda'_l,\infty)$, and applies Axiom~4 to restrict $\delta$. If $\delta$ is included in $[\lambda_l,\lambda_r]$ (applying Axiom~1 in Line~\ref{ln:implies} and checking if $(X[t], \delta) \models \sigma$), then $\Sigma$ implies $\sigma$. %if the latter is implies by $(X[t], \delta)$.  
Algorithm~\ref{alg:implies} runs in linear time w.r.t. |$\Sigma$|, and proves the implication problem can be solved in linear time.

\begin{algorithm}[tb]
%\KwIn{Set of diversity constraints $\Sigma$, and constraint $\sigma=(X[t], \lambda_l, \lambda_r) \not\in \Sigma$ over relation $R$.}
\KwOut{$\Sigma \models \sigma$.}
$\delta:=[0, +\infty)$;\label{ln:infty}\\
\ForEach{$\sigma'=(X'[t'], \lambda'_l,\lambda'_r) \in \Sigma$}{
\lIf{$X'[t'] = X[t]$}{$\delta := \delta \cap [\lambda'_l, \lambda'_r]$\label{ln:intersect}}
\lIf{$X \subset X'$ {\bf and} $t \subset t'$}{$\delta := \delta \cap [0, \lambda'_r]$\label{ln:right}}
\lIf{$X' \subset X$ {\bf and} $t' \subset t$}{$\delta := \delta \cap [\lambda'_l, +\infty)$\label{ln:left}}
}
\KwRet{$\delta \subseteq [\lambda_l,\lambda_r]$};\label{ln:implies}
\caption{\nit{Implies} ($\Sigma, \sigma=(X[t], \lambda_l, \lambda_r)$)}\label{alg:implies}
\end{algorithm}


\begin{example} \label{ex:imply} Consider the following execution of Algorithm~\ref{alg:implies} to check whether $\Sigma \models \sigma$, where $\Sigma = \{\sigma', \sigma''\}$,  $\sigma'=(\att{CTY}[\val{Calgary}], 2, 10)$, $\sigma''=(\{\att{GEN},\att{ETH},\att{CTY}\}[\val{Female},$ \ $\val{Caucasian},\val{Calgary}], 4, 7)$, and  $\sigma=(\{\att{ETH},\att{CTY}\}[\val{Caucasian},\val{Calgary}], 5, 8)$.  The range $\delta$ first reduces to $[0,10]$, and then to $[4,10]$ after considering $\sigma'$ and $\sigma''$. Line~\ref{ln:implies} returns true since $[5,8] \subseteq [4,10]$, and thus, $\Sigma$ implies $\sigma$.\boxtheorem\end{example}

\subsection{Satisfiability}\label{sec:satisfy}
{\em The satisfiability problem} is to determine whether a set of constraints $\Sigma$ is {\em satisfiable}, i.e. does there exist a relation $R$ such that $R \models \Sigma$.  We can apply Axioms 1 - 4, and test whether $\Sigma$ implies the false diversity constraint $\phi$, i.e.,  $\phi = (X[t], \lambda_l, \lambda_r)$ with empty range $[\lambda_l, \lambda_r]=\emptyset$.  Since there is no relation $R$ that satisfies $\phi$, if we infer that $\Sigma \models \phi$, then there is no $R$ that satisfies $\Sigma$, and $\Sigma$ is not satisfiable.


\begin{example} Let $\Sigma=\{\sigma',\sigma''\}$, where $\sigma'=(\{\att{ETH},\att{CTY}\}$ \\ $[\val{Caucasian},\val{Calgary}], 6, 8)$ and $\sigma''=(\att{CTY}[\val{Calgary}], 1, 5)$.  Clearly, $\Sigma$ is unsatisfiable since the target ranges are not compatible for persons from Calgary.  From Algorithm~\ref{alg:implies}, we can check that $\Sigma$ implies the false constraint $\phi = (\att{CTY}[\val{Calgary}], \emptyset)$, where $\delta = \emptyset$.  Given this, we conclude that $\Sigma$ implies $\phi$, and $\Sigma$ is not satisfiable.\boxtheorem\end{example}

\subsection{Minimal Cover}\label{sec:minimal}
To avoid redundancy, it is preferable to have a {\em minimal} set of constraints that are equivalent to $\Sigma$, i.e. a {\em minimal cover} of $\Sigma$. 

\begin{definition}\emph{(Minimal Cover)}. \label{defn:mincover}
Given two sets of diversity constraints, $\Sigma$ and $\Sigma'$, we say $\Sigma'$ {\em covers} $\Sigma$, 
if for every constraint $\sigma \in \Sigma$, $\Sigma' \models \sigma$.  A {\em minimal cover} $\Sigma'$  of $\Sigma$, is a set of diversity constraints such that $\Sigma'$ covers $\Sigma$, and there is no subset of $\Sigma'$ that covers $\Sigma$.
\end{definition}

Intuitively, a set of constraints $\Sigma'$ is minimal if every constraint $\sigma' \in \Sigma'$ is necessary.  That is, there is no constraint in $\Sigma'$ such that $\Sigma' \setminus \{\sigma'\} \models \sigma'$. In  Example~\ref{ex:imply}, the set of constraints $\Sigma=\{\sigma',\sigma''\}$ is minimal since neither $\{\sigma'\} \not\models \sigma''$ nor $\{\sigma''\} \not\models \sigma'$. However, $\Sigma \cup \{\sigma\}$ is not minimal since $\{\sigma',\sigma''\} \models \sigma$ and $\sigma$ is redundant.  We can check the minimality of a set of constraints $\Sigma$ using Algorithm~\ref{alg:implies}, by testing the logical implication of every constraint in $\Sigma$. 

%Using the notion of logical implication, we define a minimal set of diversity constraints that has no redundant constraint, i.e. a constraint that is implied by the other constraints in the set of constraints.

In the remainder of the paper, we assume $\Sigma$ is satisfiable and minimal. We verify and reject unsatisfiable sets of constraints, and verify minimality by removing redundant constraints.

\subsection{$(k,\Sigma)$-Anonymization: Decision Problem} \label{sec:anon}

%\mostafa{I think using the term satisfiability here can be confusing with satisfiability in sec 3.3.}
We now turn to the decision problem of $(k,\Sigma)$-anonymization, and show that the decision problem is tractable but unfortunately, the problem in Defn~\ref{df:k-sigma} is not. First, given our updated Defn.~\ref{df:div} of diversity constraints, we update $\Sigma$ in our $(k,\Sigma)$-anonymization problem statement in Defn~\ref{df:k-sigma} to reflect these constraints.  

\eat{ %already defined in Sec. 2. end
Now we use diversity constraints to represent diversity in data anonymization and data publishing. We define the $(k,\Sigma)$-anonymization problem that considers diversity constraints $\Sigma$.

\begin{definition}[$(k,\Sigma)$-anonymization] \label{df:pr} Consider a relation $R$ of schema $\mc{R}$, a constant $k$, a set of diversity constraints $\Sigma$. The $(k,\Sigma)$-anonymization problem is to find a relation $R^*$ that has the following properties: (1) $R \sqsubseteq R^*$, (2) $R^*$ is $k$-anonymous, (3) $R^* \models \Sigma$, and (4) $R^*$ has minimal information loss, i.e., minimum number of $\star$'s. 
\boxtheorem\end{definition}
}

\starter{The Decision Problem.}
Given relation $R$, value $k$, diversity constraints $\Sigma$, the $(k,\Sigma)$-\emph{anonymization decision problem} is to decide whether there exists an $R^*$ such that:  (1) $R \sqsubseteq R^*$; (2) $R^*$ is $k$-anonymous; and (3) $R^* \models \Sigma$.

We assume for any constraint $\sigma=(X[t], \lambda_l, \lambda_r)$ in $\Sigma$, $\lambda_l \ge k$. Constraint $\sigma$ can only be satisfied when the frequency of value $a$ is greater than or equal to $k$ due to the $k$-anonymity condition in $R^*$.

\begin{theorem}\label{th:ptime}
Consider relation $R$, value $k$, and a constraints $\Sigma$. The $(k,\Sigma)$-anonymization decision problem is in PTIME w.r.t. \eat{the size of}$|R|$.\boxtheorem\end{theorem}

\emph{Proof Sketch.} The proof of Theorem~\ref{th:ptime} is based on a naive algorithm that exhaustively checks every possible clustering of tuples in $R$ to generate $X$-groups that satisfy $\Sigma$. Since the number of possible clusterings is polynomial in the size of $R$, and exponential in the size of $\Sigma$, the decision problem is tractable. In Section~\ref{sec:alg}, we propose an algorithm for solving the $(k,\Sigma)$-anonymization decision problem by optimizing the naive algorithm, i.e., our new algorithm generates a $k$-anonymized instance $R^*$ that satisfies $\Sigma$.
 
\begin{proposition} \label{pr:np} Consider relation $R$, value $k$, and constraints $\Sigma$. The $(k,\Sigma)$-anonymization problem is NP-hard w.r.t. $|R|$.\boxtheorem\end{proposition}

\emph{Proof Sketch.} The $(k,\Sigma)$-anonymization problem extends the $k$-anonymization problem, which is proved to be NP-hard~\cite{bng-fung}\ignore{meyerson}.




%We study three fundamental problems for diversity (+ fairness?) constraints $\Sigma$: (1) \emph{satisfiability}: whether $\Sigma$ can be satisfied by an instance $R$; (2) \emph{validation}: whether a given $\sigma$ satisfies $\Sigma$; and (3) \emph{implication}: given $\Sigma$ and $\sigma \not \in \Sigma$, determine whether $\Sigma \models \sigma$.  Recall we consider two types of diversity constraints: 

%\noindent \textbf{Fixed-Bound Constraints.} 

%\noindent \textbf{Variable Bound Constraints.}  Here, we extend the diversity constrains with value suppression by allowing ceiling and floor to depend on several other values unlike Definition~\ref{df:div} that uses fixed floor and ceiling.

%\begin{definition} \label{df:div-var} Given a relation $R$ with schema $\mc{R}$ and an anonymized relation $R'$ obtained from $R$ by value suppression, a constraint with is of the following form $\nit{Floor}(...)\le A_i(a) \le \nit{Ceil}(...)$ in which $\nit{Floor}(...)$ and $\nit{Ceiling}(...)$ are functions of the number of tuples in $R$, the number of tuples $t$ in $R'$ s.t. $t[A]\neq \star$, and the number of tuples s.t. $t[A]=a$. Relation $R'$ satisfies $\sigma$, denoted by $R' \models \sigma$, if $|R'[A=a])|$ is in the range specified by $\nit{Floor}(...)$ and $\nit{Ceiling}(...)$. \end{definition}

%****************************


%We show in Section~\ref{sec:alg} that the $(k,\Sigma)$-anonymization decision problem is in PTIME when the number of constraints $|\Sigma|$, the \nit{floor} and \nit{ceil} in $\Sigma$, and the number of attributes in $\mc{R}$ are all fixed. We propose an $O(\log k)$-approximation algorithm that first answers the $(k,\Sigma)$-anonymization decision problem. If there exists an $R^*$, we present an algorithm that finds a relation $R'$ with an $O(\log k)$-approximation guarantee of information loss. 

%\begin{theorem}The satisfiability problem for $(k,\Sigma)$-anonymization is in NP-hard if $\Sigma$ includes variable-bound diversity constraints.\boxtheorem\end{theorem}

%*****************************
%\subsection{Validation}

%*****************************
\ignore{\subsection{Implication}
Consider $\sigma = (R[X], \lambda_l, \lambda_r)$ where ($\lambda_l, \lambda_r$) define the left and right frequency bounds, and $R[X]$ a  set of attribute values. We define two cases when given $R$ satisfies $\sigma$, denoted as $R \models \sigma$, we can infer diversity constraint $\sigma'$ such that $R \models \sigma'$.



\noindent \textbf{Type-1 (Fixed bounds).}  Given $\sigma = (R[X], \lambda_l, \lambda_r)$ and $\sigma' = (R[X'], \lambda_l', \lambda_r')$, where $\lambda_l  = \lambda_l'$ and $\lambda_r = \lambda_r'$.  If $R[X'] \subseteq R[X]$ and $R \models \sigma$, then $R \models \sigma'$.  Intuitively, for a fixed set of bounds, any diversity constraint $\sigma'$ with attribute values that are a subset of values in a satisfied $\sigma$ will also hold, i.e., the set of satisfying tuples will be a subset of the original set of satisfying tuples w.r.t. $\sigma$.

\noindent \textbf{Type-2 (Fixed attribute values).} Given $\sigma = (R[X], \lambda_l, \lambda_r)$ and $\sigma' = (R'[X], \lambda_l', \lambda_r')$, where $R[X] = R[X']$.  If $\lambda_l' \geq \lambda_l$ and $\lambda_r' \leq \lambda_r$ and $R \models \sigma$, then $R \models \sigma'$.   Intuitively, for a fixed set of attribute values, the set of satisfying tuples w.r.t $\sigma'$ will be a subset of those w.r.t. $\sigma$ due to the more restrictive bounds from $\sigma'$.

%In general, given a set $\Sigma$ of diversity constraints, and a diversity constraint $\sigma$, we say $\Sigma$ \emph{implies} $\sigma$, denoted as $\Sigma \models \sigma$, if $R \models \Sigma$ then $R \models \sigma$.  
Given a finite set of diversity constraints $\Sigma \cup \sigma$, the \emph{implication problem} is to determine whether $\Sigma \models \sigma$.}

%Similarly, let $\sigma' \in \Sigma$, $\sigma' = (X', \lambda_l', \lambda_r')$.  For a database instance $R$, we say that $\sigma$ \emph{implies} $\sigma'$, denoted as 
%that increases these bounds from $\sigma$, i.e., $\lambda_l' \geq \lambda_l$ and $\lambda_r' \leq \lambda_r$, the tuples matching $\sigma'$ are a subset of the tuples matched by $\sigma$.  Similarly, if we fix the bounds and vary X, 

==> problem.tex <==
\section{The $(k,\Sigma)$-Anonymization Problem}\label{sec:problem}

To capture diversity, we define a set of declarative \emph{diversity constraints} that specify lower and upper bounds on the number of attribute values in a published relation. 


%\begin{itemize}
 %   \item Fixed bound: \red{$\att{CITY}:3\le \val{Calgary} \le 12$ or $3\le \att{CITY}[\val{Calgary}] \le 12$}
    %\item Variable bound: \red{$\att{CITY}:c(..)\le \val{Calgary} \le f(...)$}
%\end{itemize}




%\vspace{2mm} \noindent \textbf{Diversity Constraints.} Diversity in an anonymised instance requires the anonymized relation to have a minimum or a maximum representation of some specific group of individuals. For example, a data publisher may prefer a $3$-anonymous relation with geographical diversity containing at least $3$ and at most $12$ patients from \val{Calgary}. We represent this with a {\em fixed-bound diversity} constraint where the minimum and maximum number of values are captured by {\em ceiling} and {\em floor} as fixed multiple of $k$, e.g. $3\le \att{CTY}(\val{Calgary})\le 12$.  In different application, the ceiling and lower bounds in a diversity constraint are often not a fixed number and depend on the total number of revealed value (non-$\star$). For example, a diversity constraint requires between $45\%$ and $55\%$ of the revealed gender values to be \val{Female}. Note that the number of revealed genders is not a fixed and known number. We capture this constraint with {\em variable-bound diversity constraints}, e.g. $0.45 \times c \le \att{GEN}(\val{Female})\le 0.55\times c$ in which $c$ is the number of non-$\star$ values in the published relation. 


To express these constraints, we adopt the definition of diversity constraints in~\cite{fairness} for relational data. In~\cite{fairness}, diversity constraints are used for {\em the set selection problem} that require diverse values among a selected set of top-$m$ items. 

%They propose these constraints for selecting items with diverse attribute values in the set selection problem, i.e. the problem of selecting top $m$ items based on some score. We adapt these constraints for attributes in relational data.

\begin{definition} [Diversity Constraints] \label{df:div} Consider a $k$-anonymous relation $R'$ with schema $\mc{R}$. We define two types of diversity constraints (the latter is a more general form of the former):

\begin{itemize}
    \item{\bf Fixed-bound constraint}: a fixed-bound constraint is of the form $\nit{floor} \le \nit{count}(R'[A],a) \le \nit{ceiling}$ in which $A \in \mc{R}$, $a \in \nit{dom}(A)$, $\nit{count}(R'[A],a)$ is the number of times the value ``$a$'' appears in $R'[A]$, and \nit{floor} and \nit{ceiling} are multiples of $k$.
    \fei{Why tie the lower and upper bound to k-anonymity? I'm hesitant to do this as it limits its general applicability.}
    \mostafa{This is not really a limitation and is only for making constraints more clear. For example, if $k=3$ then $2 \le \nit{count}(R'[A],a) \le 7$ and $1 \le \nit{count}(R'[A],a) \le 8$ have the same effect as $3 \le \nit{count}(R'[A],a) \le 6$ because $\nit{count}(R'[A],a)$ is a multiple of $k$ anyways and can not be 2, 7 and 8.}
    \fei{I understand.  However, this is assuming that the revealed values are only in QI attributes (a restriction of k-anonymity), and that each cluster is exactly size $k$.  If I have a minimum cluster size of $k$, can I not get values in $R'$ that are non-multiples of $k$?}
    
    \item{\bf Variable-bound diversity constraint}: a variable-bound diversity constraint is of the form $f(...) \le \nit{count}(R'[A],a) \le c(...)$ in which $c(...)$ and $f(...)$ are functions of $|R'|$ (the number of tuples in $R'$) and $\nit{count}(R'[A],\star)$ (the number of $\star$'s in $R'[A]$), and return multiples of $k$.
\end{itemize} A diversity constraint $\sigma$, fixed- or variable-bound, is satisfied by $R'$ denoted by $R' \models \sigma$ if and only if $\sigma$ holds as a mathematical inequality according to the attribute values in $R'$.\boxtheorem\end{definition}  

The bounds in diversity constraints enables us to specify anonymized relations with diverse values. These constraints impact the anonymization process to generate these diverse values. Clearly, this is only possible if the initial relation contains diverse values which means the diversity constraints are only indirectly affected by the initial relation; they impose restrictions solely on the anonymized relation.  Variable-bound constraints extend fixed-bound constraints by allowing bounds that depend on the total number of anonymized values ($\star$'s) and revealed values (non-$\star$'s). These are not fixed and can change during the anonymization process and therefor can not be expressed with fixed-bound constraints.
%\fei{Let's discuss: a(A), $\phi$ to $\sigma$, extension? similar notation as [5]?}

\begin{example}\em \label{ex:div} In Example~\ref{ex:intro}, $\sigma_1: 3 \le \nit{count}(R_1[\att{ETH}], \val{Asian}) \le 6$ is a fixed-bound diversity constraint over $R_1$ that requires at least 3 and at most 6 tuples with \val{Asian} ethnicity and is falsified by $R_1$ in Table~\ref{tab:r1} because there is no such ethnicity in $R_1$. A similar constraint $3 \le \nit{count}(R_2[\att{ETH}], \val{Asian}) \le 6$ is satisfied by $R_2$ in Table~\ref{tab:r2} that contains exactly $3$ Asians. A diversity constraint might have a missing upper or lower bound. For example, $3 \le \nit{count}(R_1[\att{ETH}], \val{Asian})$ is a valid diversity constraint that requires $R_1$ to have at least 3 Asians and does not impose an upper bound.

The following is a variable-bound diversity constraint that requires at least $30\%$ of the revealed genders in $R_1$ to be females: $\nit{f}(...) \le \nit{count}(R_1[\att{GEN}],$\ $\val{Female})$ with $\nit{f}(...)=\ceil{0.3 \times |R_1|-\nit{count}(R_1[\att{GEN}],\star)}_k$ ($\ceil{x}_k$ rounds $x$ to the first greater multiple of $k$, e.g. $\ceil{0.9}_3=3$ and $\ceil{4.9}_3=6$). $R_1$ falsifies the constraint because $f(...) = \ceil{0.3 \times 9 - 6}_3 = \ceil{0.9}_3 = 3$ and $R_1$ does not contain any female. Note that $|R_1|-\nit{count}(R_1[\att{GEN}],\star)$ is the number of tuples with a revealed gender value. $R_2$ in Table~\ref{tab:r2} satisfies a similar diversity constraint because it contains three females.

Diversity constraints can be extended to multiple attributes, e.g. $3 \le \nit{count}(R_2[\att{GEN},\att{ETH}],(\val{Female},\val{Asian}))$ is a fixed-bound diversity constraint that requires at least $3$ Asian females in $R_2$. Here,  $\nit{count}(R_2[\att{GEN},\att{ETH}],$ \ $(\val{Female},\val{Asian}))$ counts the number of times \val{Female} and \val{Asian} co-occur in the same tuple in $R_2$.\boxtheorem\end{example}
%restrict to least 3 and at most 4 females, and at least 3 and at most 5 African individuals

%\noindent \textbf{Problem Definition.}  We now formally define our problem.
%that finds a $k$-anonymous instance satisfying a set of diversity constraints $\Sigma$.

\vspace{2mm}
%\noindent {\bf Fairness Constraints.} The notion of fairness, as we briefly explained in Example~\ref{ex:intro}, is essentially different from diversity. The diversity constraints in Definition~\ref{df:div} are defined for an anonymized relation and are independent of the initial input relation. However, fairness is about the closeness of the distribution of values in the input relation and the anonymized output relation. For example, a data publisher might want the same ratio of female to male in the anonymized relation and the input relation. To define these fairness semantics in PPDP, we adapt the fairness constraints for set selection~\cite{fairness}.

\begin{definition} [Fairness Constraints] \label{df:div} Consider a relation $R$ with schema $\mc{R}$ and a $k$-anonymous relation $R'$ with the same schema such that $R\sqsubseteq R'$. A {\em fairness constraint} is of the form $\eta: \nit{f}(...) \le \nit{count}(R[A],a) \le \nit{c}(...)$ in which $\nit{f}(...)$ and $\nit{c}(...)$ are functions of $|R'|$, $\nit{count}(R'[A],\star)$ and $\nit{count}(R[A], a)$. $\langle R, R'\rangle\models \eta$ when $\eta$ holds as an inequality considering the values in $R$ and $R'$.\boxtheorem\end{definition}  

Fairness constraints extend variable-bound constraints by allowing bounds that depend not only on anonymized relation $R'$ but also the initial relation $R$ (in particular $\nit{count}(R[A],a)$). This enables the fairness constraints to compare the distribution of values in the two relations. Fairness, as a general requirement, is usually interpreted as having an anonymized relation with similar distribution of values to the distribution of values in the initial relation. This can be expressed by the fairness constraints.

\begin{example} The fairness constraint $f(...) \le \nit{count}(R_2[\att{GEN}],$ \ $\val{Female})$ with $f(...)=\ceil{p \times (|R_2|-\nit{count}(R_2[\att{GEN}],\star)}_3$ requires at least $p\%$ of the revealed genders in $R_2$ to be \val{Female} in which $p$ is the percentage of females in the initial relation $R$ (note that $|R|=|R_2|$):  

\vspace{-3mm}
\begin{align*}p=\frac{\nit{count}(R[\att{GEN}], \val{Female})}{|R|}\end{align*}

\noindent According to the data of $R$ and $R_2$ in Tables~\ref{tab:r} and \ref{tab:r2}, resp., $\langle R,R_2 \rangle$ satisfy this fairness constraint. That is because $f(...)=\ceil{4/9 \times (9 - 6)}_3=\ceil{4/9 \times (9 - 6)}_3=3$ and there are exactly $3$ females in $R_2$.\boxtheorem\end{example}

\noindent \textbf{Problem Statement.} 
\begin{definition}[$(k,\Sigma)$-anonymization] \label{df:pr} Consider a relation $R$ of schema $\mc{R}$, a constant $k$, a set of constraints $\Sigma=\Sigma_1\cup\Sigma_2$ with diversity constraints $\Sigma_1$ and fairness constraints $\Sigma_2$. The {\bf $(k,\Sigma)$-anonymization problem} is to find a relation $R^*$ that has the following properties: (1) $R \sqsubseteq R^*$, (2) $R^*$ is $k$-anonymous, (3) $R^* \models \Sigma_1$, (4) $\langle R, R^*\rangle \models \Sigma_2$, and (5) $R^*$ has minimal information loss, i.e., minimum number of $\star$'s.
\boxtheorem\end{definition}


\noindent \textbf{Complexity Analysis.} 
The $(k,\Sigma)$-anonymization problem is NP-hard because it generalizes the $k$-anonymization problem with diversity and fairness constraints in $\Sigma$. 
%The following theorems prove the complexity of the satisfiability problem for $(k,\Sigma)$-anonymization.  



%\fei{The last part of this sentence sounds as if we are just adopting an existing algorithm [14], with little novelty.  Can we re-phrase this to sound more novel?}

%\begin{proposition} The $(k,\Sigma)$-anonymization problem is NP-hard and the $(k,\Sigma)$-anonymization decision problem is in PTIME.\end{proposition}

 %\fei{sub-optimal, can we be more specific, does not sound appealing}

\ignore{\begin{table}[h]
\begin{center}
\normalsize
\setlength\tabcolsep{2 pt}
\vspace{-3mm}
%\scalebox{0.9}{
\begin{tabular}{ | l | l | l | l || l | l | l |}
\hline
 \textbf{ID}  &  \textbf{PC}    &  \textbf{PRV} &  \textbf{GEN} &  \textbf{DIAG} &  \textbf{MED}  \\
\hline \hline
$t_1$  &   {\bf R7A} &  {\bf AB} & *  &  {Osteoarthritis} & {Ibuprofen}\\
\hline
$t_2$  &   {\bf R7A} & {\bf AB} & * &  {Osteoarthritis} & {Naproxin}\\
\hline
%$t_5$  &   K2H & ON & Female &  seizure & diazepam\\ \hline
%$t_6$  &    J5B & QC & Female &  seizure & diazepam\\ \hline
$t_3$  &    {\bf R7A}  & {\bf MB} & * &  {Osteoarthritis} & {Naproxin}\\
\hline
$t_4$  &    {\bf R7A}  & {\bf MB} & * &  {Osteoarthritis} & {Ibuprofen}\\
\hline
$t_6$  &    J5B & QC & {\bf Male} & {\bf Seizure} & {\bf Diazepam}\\
\hline
$t_7$  &    J5B & QC & {\bf Male} & {\bf Seizure} & {\bf Digoxin}\\
\hline
\end{tabular}
\vspace{0mm}
\caption{General and inconsistent relation $R_1$}
\label{tab:r1}
\end{center}
\end{table}}

\ignore{\begin{figure}[h]
\begin{center}
%\vspace*{-4mm}
\includegraphics[width=7cm]{./figs/figs.pdf}
%\vspace*{-4mm}
\caption{\vghs of (a) PRV and (b) MED.}\label{fig:general}
\end{center}
\end{figure}}

\ignore{A private relation in PPDP can be subject to some integrity constraints (ICs) to keep its data consistent. These constrains might be falsified by the private relation for different reasons such as the integration of data from conflicting sources, faulty data entry, or data staleness. In $R$, we assume two simple ICs in form of FDs $\varphi_{1}: \nit{PC} \rightarrow \nit{PRV}$ and $\varphi_{2}: [\nit{GEN},\nit{DIAG}] \rightarrow \nit{MED}$ that are falsified by $t_1$-$t_4$ and $t_7,t_8$, respectively (error values in bold). A public general relation in PPDP might inherit this inconsistency from its private relation as this happened in $R_1$. In this work, we would like to define the data consistency in the public relation as the third objective in PPDP.}

\ignore{\begin{table}[h]
\begin{center}
\normalsize
\setlength\tabcolsep{2 pt}
%\scalebox{0.9}{
\begin{tabular}{ | l | l | l | l || l | l | l |}
\hline
 \textbf{ID}  &  \textbf{PC}    &  \textbf{PRV} &  \textbf{GEN} &  \textbf{DIAG} &  \textbf{MED}  \\
\hline \hline
$t_1$  &   R7A &  Prairies & Female  &  {Osteoarthritis} & {Ibuprofen}\\
\hline
$t_2$  & R7A & Prairies & Male &  {Osteoarthritis} & {Naproxin}\\
\hline
%$t_5$  &   K2H & ON & Female &  seizure & diazepam\\ \hline
%$t_6$  &    J5B & QC & Female &  seizure & diazepam\\ \hline
$t_3$  & R7A & Prairies & Male &  {Osteoarthritis} & {Naproxin}\\
\hline
$t_4$  & R7A & Prairies & Female &  {Osteoarthritis} & {Ibuprofen}\\
\hline
$t_6$  &    J5B & QC & Male & Seizure & Anesthetics\\
\hline
$t_7$  &    J5B & QC & Male & Seizure & Anesthetics\\
\hline
               \end{tabular}
\caption{\small General and consistent relation $R'$}
\label{tab:r2}
\end{center}
\end{table}}

\ignore{To publish a consistent version of an inconsistent private relation, we can repair the relation before publishing it. However, it might be preferable to integrate data repair with the data generalization process. This is mainly because data repair is usually costly and it can only be applied to a limited number of errors in an error prune and inconsistent private relation while some of the repaired values might be generalized and detracted in the generalization process for data publishing. For example, $R_2$ in Table~\ref{tab:r1} is a public $k$-anonymous version of $R$ that generalizes AB and MB to Prairies. If we decide to publish $R_2$ there is no point in repairing $t_1$-$t_4$ by updating AB to MB which might be expensive to figure out while it will be distorted anyway during the generalization process. This generalization masks the violation of $\sigma_1$ and it can be seen as a form of data repair.  This basically shows by integrating data repair and the generalization process, we have to ways to resolve inconsistency in a private relation, either by repairing them (e.g. AB to MB in case we decide to publish $R_1$) or by masking the errors thought value generalization. Assuming a limited resources for data repair, we can balance between these two to obtain a consistent and general relation. For example, if there is only one value repair can be done in $R$, we can resolve errors in $t_1$-$t_4$ through generalization and save this repair to fix $t_6$, e.g. Diazepam to Diagoxin which will not be detracted and will be published.  }

\ignore{Based on the discussion above, we define the problem of consistent data publishing as follows. Consider a relation $R$ of schema $\mc{S}$ with a set of QIs $A_1,...,A_n$ and sensitives $B_1,...,B_m$ and a set of FDs $\Sigma$. Let $\nit{cost}_\Sigma(.)$ be a function that specifies the cost of repairing a relation of schema $\mc{S}$ w.r.t. $\Sigma$, $\nit{loss}(.)$ be function that measures of information loss in a relation of $\mc{S}$, and let $B$ be a fixed repair budget. The problem is to find a public relation $R'$ of schema $\mc{S}$ that satisfies the followings: 

\begin{enumerate}
    \item $R'$ generalizes $R$,
    \item it is $k$-anonymous,
    \item $\nit{cost}_\Sigma(R') \le B$,
    \item $R'$ has minimum $\nit{loss}( R')$.
\end{enumerate}}

%\mostafa{Here I defined the problem using a single cost function and not a cost model for each repair operation. I did this because I did not want to get involved with how repair is done and what repair operations are.}


%\fei{Or as we discussed, it may just mask an error, which may not be satisfactory either.} \mostafa{We can cite~\cite{solmaz} as a similar repair technique to justify this way of repair.} 

%Third, the usefulness of the repaired values in a private relation depends on the accuracy of the applied repair algorithms. For example, a repair algorithm might update MB in $t_3$ and $t_4$ to AB to resolve the inconsistency while we know R7A is actually a postal code in MB. These are reasons that someone might choose $R_2$ that resolves the FD violation by generalization rather than application of a separate repair algorithm.  \fei{Yes, but this point requires known semantics between PC and PRV, which we are not providing in this proposed work right?  There is a fundamental assumption here that the dirty data values are somewhat close, albeit inconsistent, in order for your Prairies repair to work.  If the dirty data values are ``far apart'' then generalization does not provide added value.}

%\fei{I would add a point that given limited cleaning resources, it is not always possible to clean a large number of cells, we must be selective due to finite resources, which we can model via a budget.} 
%\blue{This might have different reasons. First, the repair algorithms usually have limited cleaning resources and can not repair large number of cells and therefore it might not be possible to repair every cell in a private database.}  Second, repairing some values might be redundant if they are generalized in the generalization step. 



%\mostafa{If by semantics you mean the semantics encoded in the generalization hierarchies, I think it is reasonable to assume we have these hierarchies. About close vs far values to be repaired and having added value, there is no real added information here. Even when two dirty values are close, repairing them to their least common ancestor causes loss of information, however it will also resolves inconsistency. Basically, here any repair will cause information loss, if value are further apart (meaning the data is dirtier) more generalization is needed to mask the inconsistency.}


%\fei{Like we discussed, we need to add discussion re. differential privacy and privateClean and distinctions.}

%\mostafa{I added sentences after the problem definition. I think these are different problems although both are about privacy and cleaning.}

%In $R_2$, generalization achieves both the $k$-anonymity privacy requirement and data consistency. In particular, the generalization of Diazepam and Digoxin only resolves the inconsistency w.r.t. $\sigma_2$ and is not necessary for $k$-anonymity. The generalization of AB and MB helps to satisfy $k$-anonymity and the violation of $\sigma_1$. 




%Generalization can also facilitate data repair by transforming inconsistent values to less specific but semantically close values according to a domain generalization hierarchy. In our example, we can generalize $R$ to $R''$ the PRV values in tuples $t_1, t_2, t_7, t_8$ by generalizing the existing values to `Prairies' according to the PRV domain hierarchy shown in  Figure~\ref{fig:general}(a). 


%Example~\ref{ex:k} shows that generalization can serve for both privacy preservation and data repair by masking inconsistencies. Here, we define the problem of clean data publishing to achieve both of these two objectives. For a relation $R$, a set of ICs $\Sigma$ that are falsified by $R$ ($R\not\models \Sigma$), and value $k$ as in $k$-anonymity, the problem of clean data publishing is to find a relation $R'$ that (1) satisfies $\Sigma$, (2) is $k$-anonymous, and (3) minimally generalizes $R$. Here, (1) and (2) concern data consistency and privacy, while (3) restricts the amount of change applied on the given relation $R$ which is a common objective in both data publishing and data repair. The instance $R_2$ in Example~\ref{ex:k} is a possible solution of the problem.

%\blue{PrivateClean is a data cleaning framework addressing a similar problem~\cite{krishnan}. It cleans a differentially private version of the underlying private database that contains dirty values using a limited set of cleaning operations. PrivateClean is different from our problem of clean data publishing. In PrivateClean date repir is delayed and is done over private versions of the original relations. However, here we integrate both cleaning and privacy-aware data publishing in a single task to get higher utility in the result of cleaning. Second, PrivateClean assumes the cleaning process is unknown and only allows a limited cleaning operations that might be used in this process. In our problem, there might be many existing cleaning algorithms that we decide not to apply for the reasons we mentioned in Example~\ref{ex:k}. Finally, the privacy models are different and the differentially private restriction in PrivateClean does not allow high utility cleaning algorithms to run over the private data.}

%\fei{I think there are two problems that need to be solved:}
%\begin{itemize}
%    \item  (i) how to first ``clean'' values that are inconsistent such that they are close and generalization will work; and (ii) deciding on which values to generalize and how much.

%\mostafa{About (i), if we can accurately repair, there is no need to mask violations using generalization. Unless we say only few values can be repaired and then we would like to find those that make generalization more efficient while generalization is still going to mask some violation that are left in the data. This requries a different problem definition with limited repair budget in the first repair phase and then a generalization step to mask errors. Is that the idea?}    

%\mostafa{About (ii), this is already encoded in problem definition. Since there are several instances that satisfy (1) and (2). While (3) captures the restriction on the values to pick for generalization and the extent of generalization over these values.}    

    %\item I think it's also worthwhile to demonstrate in the example a stronger case where by generalizing only (without consideration for cleaning) leads to a very different clustering of tuples than if we were to clean + generalize together, which is a correct solution that uses the FDs (and its semantics) to determine which cells to clean.  This probably requires QI attributes to not be part of the FD attributes.
    
    %\mostafa{I think Table~\ref{tab:r1} and Table~\ref{tab:r1} do exactly what you said. They have different clusterings but Table~\ref{tab:r1} applies cleaning+generalization while Table~\ref{tab:r1} does not clean data beforehand. I did not talk about clustering since it is not part of problem definition and it is about solution.}
%\end{itemize}


==> tableExtra.tex <==







\begin{table}[htbp]
    \centering
    \Large
    \resizebox{\linewidth}{!}{
\begin{tabular}{l@{\hskip 0.048in}c@{\hskip 0.048in}c@{\hskip 0.048in}c@{\hskip 0.048in}c@{\hskip 0.048in}c@{\hskip 0.048in}c@{\hskip 0.048in}c}
    \toprule
Model & { \amzgog} & { \walamz} & { \DBLPGogS} & { \DBLPACM} & { \Beer} & { \FodorZag} & { \itunamz} \\
    \midrule




\stdBlock & 
\underline{1.7}, \large{98.4} &
1.5, \large{99.2} &
0.8, \large{98.8} &
-0.2, \large{99.8} &
\underline{-1.7}, \large{94.9} &
\bestnumber{0}, \large{100} &
7.5, \large{100} \\

\qgram & 
\bestnumber{-1.0}, \large{95.7} &
1.5, \large{99.2} &
1.3, \large{98.6} &
\bestnumber{-0.05}, \large{99.95} &
-6.8, \large{89.7} &
\bestnumber{0}, \large{100} &
\fboxcolor{-9.4}, \large{70.7} \\

\exQgram & 
6.2, \large{94.5} &
\underline{1.1}, \large{98.9} &
1.2, \large{97.7} &
\bestnumber{-0.05}, \large{99.95} &
\fboxcolor{-9.4}, \large{87.2} &
\bestnumber{0}, \large{100} &
\bestnumber{-0.8}, \large{71.7} \\

\suffix & 
16.0, \large{89.3} &
5.3, \large{91.7} &
\bestnumber{0.3}, \large{82.4} &
\underline{-0.1}, \large{99.9} &
-8.5, \large{84.6} &
\bestnumber{0}, \large{100} &
\underline{1.1}, \large{51.1} \\

\exSuffix & 
\fboxcolor{18.2}, \large{84.8} &
\bestnumber{0.9}, \large{88.4} &
1.7, \large{76.6} &
-0.6, \large{99.4} &
-5.9, \large{87.2} &
\underline{-3.0}, \large{97.0} &
2.2, \large{52.2} \\

\AutoBlock & 
9.0, \large{89.0} &
4.7, \large{96.8} &
-0.6, \large{95.2} &
-0.2, \large{99.8} &
\bestnumber{-1.6}, \large{84.6} &
\bestnumber{0}, \large{100} &
-7.0, \large{88.0} \\

\CTT & 
2.8, \large{96.1} &
4.8, \large{97.9} &
\underline{0.5}, \large{96.0} &
-0.2, \large{99.8} &
-4.2, \large{92.3} &
\bestnumber{0}, \large{100} &
-1.2, \large{91.3} \\

\graphblk & 
2.4, \large{94.0} &
\fboxcolor{17.3}, \large{85.5} &
\fboxcolor{-7.3}, \large{78.6} &
\fboxcolor{-1.0}, \large{98.6} &
-2.5, \large{87.2} &
\fboxcolor{-6.7}, \large{73.3} &
-4.2, \large{53.3} \\

    \bottomrule
    \end{tabular}
    }
    \caption{\PC disparities and \PC values within the minority and majority groups}
    \label{tab:pc_combined}
\end{table}














\begin{table}[htbp]
    \centering
    \Large
    \resizebox{\linewidth}{!}{
\begin{tabular}{l@{\hskip 0.048in}c@{\hskip 0.048in}c@{\hskip 0.048in}c@{\hskip 0.048in}c@{\hskip 0.048in}c@{\hskip 0.048in}c@{\hskip 0.048in}c}
    \toprule
Model & { \amzgog} & { \walamz} & { \DBLPGogS} & { \DBLPACM} & { \Beer} & { \FodorZag} & { \itunamz} \\
    \midrule
\stdBlock & 
\underline{0.9}, \large{99.1} & 
0.8, \large{99.5} & 
0.4, \large{99.4} & 
-0.1, \large{99.9} & 
\bestnumber{-0.9}, \large{97.3} & 
\bestnumber{0.01}, \large{99.36} & 
3.8, \large{99.9} \\

\qgram & 
\bestnumber{-0.3}, \large{97.7} & 
0.9, \large{99.5} & 
0.7, \large{99.3} & 
\bestnumber{-0.03}, \large{99.94} & 
-3.7, \large{94.6} & 
-0.1, \large{99.4} & 
\fboxcolor{-6.1}, \large{82.7} \\

\exQgram & 
3.5, \large{97.0} & 
\underline{0.7}, \large{99.3} & 
0.6, \large{98.8} & 
\bestnumber{-0.03}, \large{99.94} & 
\fboxcolor{-5.1}, \large{93.1} & 
-0.07, \large{99.42} & 
\bestnumber{-0.6}, \large{83.4} \\

\suffix & 
9.8, \large{94.3} & 
3.0, \large{95.6} & 
\bestnumber{0.16}, \large{90.35} & 
\underline{-0.06}, \large{99.92} & 
-4.8, \large{91.6} & 
-0.09, \large{99.64} & 
1.0, \large{67.6} \\

\exSuffix & 
\fboxcolor{11.8}, \large{91.7} & 
\bestnumber{0.5}, \large{93.9} & 
1.1, \large{86.7} & 
-0.3, \large{99.7} & 
-3.3, \large{93.1} & 
-1.6, \large{98.2} & 
1.9, \large{68.6} \\

\AutoBlock & 
5.2, \large{93.5} & 
2.5, \large{98.3} & 
-0.3, \large{97.5} & 
-0.3, \large{98.8} & 
\underline{-1.0}, \large{91.0} & 
0.6, \large{91.9} & 
-3.8, \large{93.6} \\

\CTT & 
1.4, \large{97.3} & 
2.5, \large{98.6} & 
\underline{0.24}, \large{97.92} & 
-0.2, \large{98.8} & 
-2.3, \large{95.2} & 
\underline{0.02}, \large{91.83} & 
\underline{-0.7}, \large{95.4} \\

\graphblk & 
1.4, \large{95.9} & 
\fboxcolor{11.1}, \large{91.1} & 
\fboxcolor{-3.7}, \large{87.3} & 
\fboxcolor{-0.5}, \large{99.3} & 
-1.5, \large{92.6} & 
\fboxcolor{-3.8}, \large{83.6} & 
-3.8, \large{67.0} \\
    \bottomrule
    \end{tabular}
    }
\caption{\Fb disparities and \Fb values within the minority and majority groups}
    \label{tab:fb_combined}
\end{table}
